Causal DAG Summarization (Full Version)

Causal inference aids researchers in discovering cause-and-effect relationships, leading to scientific insights. Accurate causal estimation requires identifying confounding variables to avoid false discoveries. Pearl's causal model uses causal DAGs to identify confounding variables, but incorrect DAGs can lead to unreliable causal conclusions. However, for high dimensional data, the causal DAGs are often complex beyond human verifiability. Graph summarization is a logical next step, but current methods for general-purpose graph summarization are inadequate for causal DAG summarization. This paper addresses these challenges by proposing a causal graph summarization objective that balances graph simplification for better understanding while retaining essential causal information for reliable inference. We develop an efficient greedy algorithm and show that summary causal DAGs can be directly used for inference and are more robust to misspecification of assumptions, enhancing robustness for causal inference. Experimenting with six real-life datasets, we compared our algorithm to three existing solutions, showing its effectiveness in handling high-dimensional data and its ability to generate summary DAGs that ensure both reliable causal inference and robustness against misspecifications.

==> 00-response.tex <==
\twocolumn
\section*{Response to the Reviewers}
\noindent \textbf{Dear reviewers,}

\noindent 
We would like to express our gratitude to the reviewers for their valuable feedback, which helped us improve our paper.
In response to the reviewers' comments, we focused on addressing four main areas of improvement: (1) clarifying the complexity of the problem addressed, (2) enhancing the presentation, (3) including an ablation study, and (4) clarifying our main contributions in relation to prior work.
To address these issues, we have provided a detailed explanation of our responses to the main concerns that were raised by all reviewers. We have also addressed each reviewer's comments individually.
% \anna{Somehow it hasn't occurred to me until now to consider referring to the reviewers in the second person ('you', 'yours', etc.)... and I wonder if the letter can still be formal but speak more directly/personably to the reviewers if we said something like "We would like to express our gratitude to all of you for your valuable feedback... In response to your comments, we focused on ..."}

Updates made in response to specific comments are highlighted in the revised manuscript using the following colors:
\begin{itemize}
\item \common{Changes for multiple reviewers in Orange}
\item \reva{Reviewer 1 in Blue}
\item \revb{Reviewer 2 in Magenta}
\item \revc{Reviewer 3 in Purple} 
\end{itemize}



\subsection*{Summary of the Main Changes}




% \vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{1}}) Additional Experiments}}. 
\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{1}})
% \label{rev:point-1}
Clarifying the complexity of the causal DAG summarization problem}} Following the reviewers' suggestions, we have incorporated more details regarding the NP-hardness proof into the revised paper and clarified why obtaining an algorithm with approximation guarantees is non-trivial. The main changes are summarized below:


\noindent
$\bullet$ \textbf{NP-hardness proof.}
In our previous version, we did not include intuition or key details for this proof. 
% \markos{in the main text of our paper, pushing the entire proof to our technical report}.
% Consequently, I have two suggestions for how to improve this section:
% (1) I might suggest splitting this \colorbox{pink}{Point \textrm{1}} into two points, one addressing comments on the problem specifically (where we include an abbreviated intuition for how the proof works) and one addressing comments on the algorithm specifically (where we respond to the meta-reviewer's ask for formal guarantees on the algorithm, that any algorithm will not have formal guarantees based on our NP-completeness proof).
% (1)
% I think we should succintly describe \textit{how} \probName\ is reduced from $k$-(Max?)-Cut,
% % In discussing the NP-hardness of the \probName\, I suggest we give a concise illustration for how \probName\ is reduced from an NP-complete problem,
% ideally immediately after Theorem~\ref{theorem:problem-is-np-hard}. The meta-reviewer asked directly for the NP-hardness proof; but as far as I can tell, the additional paragraph in Section~\ref{subsec:canonical_DAG}
% %addresses the NP-hardness of providing a formal guarantee by illustrating
% illustrates how we \textit{reformulated} the \probName\ problem but did not tie the reformulated problem back to any specific NP-complete problem there.
% I'm concerned the reviewers might not understand how the problem is NP-hard if we don't walk them through it with a bit more detail. (Perhaps this just means I haven't convinced myself this isn't possible yet, I can think a bit more on how this can be achieved.)
% %
% (2) When discussing the algorithm's guarantees, I suggest we take this approach to highlight the point we're making: Point out that based on the reviewers' comments, mainly \colorbox{pink}{\textbf{R1.W2 + R1.D2}} which speaks directly to this, the heuristics in the algorithm that need formal guarantees are about minimizing additional edges in the canonical causal DAG. Based on the specific optimization problem we demonstrated to be NP-complete in our proof, providing formal guarantees for minimizing additional edges is NP-hard, and therefore not possible to include.
% \anna{(lower-level suggestion to rephrase the remainder of this paragraph, if the higher-level suggestion is not taken, but didn't figure out how to fit the detail about the proof depending on edge addition \& node contraction)
In response to the reviewers' request, we now discuss our hardness proof in the paper in Section \ref{subsec:canonical_DAG}; the proof relies on the relationship between node contractions and edge addition, which we cover earlier in that same section.
Due to space limitations, we provided only an intuition rather than the full proof. We have since refined the proof and added more details. As it now spans nearly a full page, we have deferred it to our technical report~\cite{full} and omitted it from this letter for brevity.
% \anna{further, describing our reformulation of the problem in preparation of the np-hard proof with edge additions is different from giving an intuition for how the proof itself works (for example mentioning k-max-cut)... not sure what phrasing makes the most sense}

% \anna{(suggestion to help rephrase this remainder of the section since I found it a bit hard to read easily and want to ensure the reviewers agree with the change as smoothly as possible)
With our discussion in Section~\ref{subsec:canonical_DAG}, we elaborate that the NP-Hard \probName\ problem in Theorem~\ref{theorem:problem-is-np-hard} can be formulated as finding a summary DAG $(\qg,f)$ whose \groundedDAG\ $\cg_{\qg}$ results in the smallest number of added edges, namely $|\edges(\cg_{\qg})|-|\edges(G)|$.
Specifically, we demonstrate in the proof of Theorem~\ref{theorem:problem-is-np-hard} that finding a summary DAG $(\qg,f)$ of size $|\nodes(\qg)|=k$ with at most $\tau$ additional edges (written $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$ for some threshold $\tau >0$) is NP-complete.
% }
% In particular, we now explain in Section \ref{subsec:canonical_DAG} that Theorem~\ref{theorem:problem-is-np-hard} establishes that finding a summary DAG $(\qg,f)$ whose causal DAG $\cg_{\qg}$ results in the smallest number of added edges $|\edges(\cg_{\qg})|-|\edges(G)|$ is NP-Hard. Specifically, the proof of Theorem~\ref{theorem:problem-is-np-hard} shows that finding a summary DAG $(\qg,f)$ where $|\nodes(\qg)|=k$ and $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$ for some threshold $\tau >0$ is an NP-complete problem.

In fact, in our technical report~\cite{full} we go on to prove the NP-hardness of a stronger problem: finding a summary DAG $(\qg,f)$ of size $|\nodes(\qg)|=k$ and the additional edges in the \groundedDAG\ between nodes of the same cluster node are at most $\tau$:
\begin{equation}
\label{eq:specialedges1}
    \left| \set{(X_i,X_j)\in \edges(\cg_{\qg}){\setminus}\edges(G) : f(X_i)=f(X_j} \right|\leq \tau.
\end{equation}
If $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$, then~\eqref{eq:specialedges1} must hold as well. Given this relationship of the two problems, and that finding a summary DAG where~\eqref{eq:specialedges1} holds is NP-Hard, we find that finding a summary DAG where $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$ is NP-Hard as well.




% \vspace{1mm}
% For completeness of this letter, we provide here the full proof (which is also available now in the appendix of our full version \cite{full}).

% We show that the \probName\ problem is $NP$-hard via a reduction from the $k$-Max-Cut problem~\cite{DBLP:journals/tcs/GareyJS76}. Let $G$ be an undirected graph with weighted edges (i.e., $w: \nodes(G) \rightarrow \mathbb{R}_{\geq 0}$).
% The $k$-Max-Cut problem consists of
% partitioning $\nodes(G)$ into $k$ disjoint clusters so as to maximize the sum of weights
% of the edges joining vertices in different clusters. It is well-known that $k$-Max-Cut is NP-hard even if $k=2$~\cite{DBLP:journals/tcs/GareyJS76}, and the weight of every edge is $1$. In other words, deciding whether there exists a $k$-clustering of $\nodes(G)$ to clusters $\set{V_1,\dots,V_k}$, where the sum of weights of edges between vertices in distinct clusters is at least a given threshold $\gamma$ is NP-hard.

% Let $\mathcal{S}\eqdef \set{V_1,\dots,V_k}$ be a $k$-clustering of $G$. We define $M_G(\mathcal{S})$ to be the number of edges between vertices in a common cluster:
% \begin{equation}
% \label{eq:M(S)}
% M_G(\mathcal{S})\eqdef \sum_{i=1}^k \sum_{u,v\in V_i} \mathbb{1}[(u,v)\in \edges(G)].
% \end{equation}
% We define $\overline{M}_G(\mathcal{S})$ to be the number of non-edges between vertices in a common cluster:
% \begin{equation}
% \label{eq:overM(S)}
% \overline{M}_G(\mathcal{S})\eqdef \sum_{i=1}^k \sum_{u,v\in V_i} \mathbb{1}[(u,v)\notin \edges(G)].
% \end{equation}

% Similarly, we define $B_G(\mathcal{S})$ to be the number of edges between vertices in distinct clusters:
% \begin{equation}
% \label{eq:B(S)}
% B_G(\mathcal{S})\eqdef \sum_{1\leq i<j \leq k} \sum_{\substack{u\in V_i, \\v\in V_j}}\mathbb{1}[(u,v)\in \edges(G)].
% \end{equation}
% Since every edge $(u,v)\in \edges(G)$ is either between vertices in the same cluster or vertices in distinct clusters, then:
% \[
% M_G(\mathcal{S})+B_G(\mathcal{S})=|\edges(G)|.
% \]
% In particular, $M_G(\mathcal{S})\leq \tau$ if and only if $B_G(\mathcal{S})\geq |\edges(G)|-\tau$, for every $\tau\in [0,|\edges(G)|]$.

% \begin{lemma}
% \label{lem:MInimizeM(S)}
%    Let $G$ be an undirected graph, $k\geq 2$, and $\tau \in [0,|\edges(G)|]$. Deciding whether there exists a $k$-clustering $\mathcal{S}$ of $G$ such that $M_G(\mathcal{S})\leq \tau$ is NP-Complete.
% \end{lemma}
% \begin{proof}
%     The problem is clearly in NP because given a $k$-clustering $\mathcal{S}$, computing $M_G(\mathcal{S})$ (see~\eqref{eq:M(S)}) can be done in polynomial time.
    
%     We prove hardness by reduction from $k$-Max-Cut. Suppose there exists a $P$-Time algorithm that given an undirected graph $G$, and a threshold value $\tau\in [0,|\edges(G)|]$, returns a $k$-clustering $\mathcal{S}$ such that $M_G(\mathcal{S})\leq \tau$ if one exists, and null otherwise. We show that such an algorithm can be applied to solve $k$-Max-Cut in polynomial time.

%     Let $G$, $k$, and $\gamma$ be an instance of the $k$-max-Cut problem where $G$ is an undirected graph, $k\leq |\nodes(G)|$, and $\gamma\in [0,|\edges(G)|]$. We define $\tau\eqdef |\edges(G)|-\gamma$, and execute the algorithm for finding a $k$-clustering $\mathcal{S}$ such that $M_G(\mathcal{S})\leq \tau$. Since $M_G(\mathcal{S})+B_G(\mathcal{S})=|\edges(G)|$, then:
%     \begin{align*}
%         B_G(\mathcal{S})&=|\edges(G)|-M_G(\mathcal{S})&& \Rightarrow_{M_G(\mathcal{S})\leq \tau}\\
%         &\geq |\edges(G)|-\tau && \Rightarrow_{\tau \eqdef |\edges(G)|-\gamma}\\
%         &=|\edges(G)|-(|\edges(G)|-\gamma) &&\\
%         &=\gamma &&
%     \end{align*}
%    Hence, we can decide in $P$-Time whether $G$ has a $k$-cut whose cardinality is at least $\gamma$. 
% \end{proof}
% \begin{lemma}
%     \label{lem:overlineMNPHard}
%    Let $G$ be an undirected graph, $k\geq 2$, and $\tau \in [0,|\edges(G)|]$. Deciding whether there exists a $k$-clustering $\mathcal{S}$ of $G$ such that $\overline{M}_G(\mathcal{S})\leq \tau$ is NP-Complete.
% \end{lemma}
% \begin{proof}
% The problem is clearly in NP because given a $k$-clustering $\mathcal{S}$, computing $\overline{M}_G(\mathcal{S})$, and verifying $\overline{M}_G(\mathcal{S})\leq \tau$ can be done in polynomial time (see~\eqref{eq:overM(S)}).

% So, suppose that there exists a $P$-Time algorithm that given an undirected graph $G$, and a threshold value $\tau\in [0,|\edges(G)|]$, returns a $k$-clustering $\mathcal{S}$ such that $\overline{M}_G(\mathcal{S})\leq \tau$ if one exists, and null otherwise. We show that such an algorithm can be applied to decide whether there exists a $k$-clustering of $G$ where $M_G(\mathcal{S})\leq \alpha$. By Lemma~\ref{lem:MInimizeM(S)}, this problem is NP-Hard, and hence this will prove that minimizing $\overline{M}_G(\mathcal{S})$ is NP-hard as well.

% So let $G$, $k$, and $\alpha$ be the input to the problem for deciding whether there exists a $k$-clustering $\mathcal{S}$ such that $M_G(\mathcal{S})\leq \alpha$. Let $\overline{G}$ denote the complement graph of $G$. That is $\nodes(\overline{G})=\nodes(G)$ and $(u,v)\in \edges(G)$ if and only if $(u,v)\notin \edges(\overline{G})$. In particular, $\overline{M}_{\overline{G}}(\mathcal{S})=\alpha$ if and only if $M_G(\mathcal{S})=\alpha$. Therefore, if we can, in $P$-Time find a clustering that minimizes $\overline{M}_{\overline{G}}(\mathcal{S})$, then we have also found a clustering that minimizes $M_G(\mathcal{S})$. This completes the proof.
% \end{proof}

% We now show that the \probName\ problem is $NP$-hard. Specifically, we show that finding a summary DAG $(\qg,f)$ whose canonical DAG $\cg$ minimizes $|\edges(\cg_{\qg})|-|\edges(G)|$; that is, the canonical DAG $\cg_{\qg}$ results in the smallest number of added edges, is NP-Hard.
% % \begin{theorem}
% %     The \probName\ problem which minimizes the number of added edges to the canonical DAG is NP-Hard. 
% % \end{theorem}
% \begin{proof}
%     Given a DAG $D$ and a $k$-clustering $\mathcal{S}$ of $D$, it is straightforward to verify that $\overline{M}_D(\mathcal{S})\leq \tau$, and hence this problem is in NP.

%     Let $G$ be an undirected graph, $k>0$, and $\gamma>0$ a threshold. Let $\nodes(G)=\set{v_1,\dots,v_n}$ denote a complete order of $\nodes(G)$. Define $D$ to be the directed graph where $\nodes(D)=\nodes(G)$ and $(v_i\rightarrow v_j)\in \edges(D)$ if and only if $(v_u,v_j)\in \edges(G)$ and $i<j$. Let $\mathcal{S}=\set{V_1,\dots,V_k}$ be a $k$-clustering of $\nodes(D)=\nodes(G)$ such that $\overline{M}_D(\mathcal{S})\leq \gamma$. By the definition of $\edges(D)$, we immediately get that $\overline{M}_G(\mathcal{S})\leq \gamma$. 
%     By Lemma~\ref{lem:overlineMNPHard}, the \probName\ problem is $NP$-hard. 
% \end{proof}



\noindent
$\bullet$ \textbf{Explaining why the algorithm does not have theoretical guarantees}:
As explained above, % the \probName\ problem
providing formal quality guarantees for limiting the number of additional edges
is NP-hard; therefore, it is not trivial to devise an efficient algorithm with theoretical guarantees.
As we mention in the related work section (Section \ref{sec:related_work}), our algorithm 
follows a previous line of work ~\cite{tian2008efficient,geisberger2012exact}, where a bottom-up greedy approach is used to identify promising node pairs for contraction, similar to the K-Snap algorithm~\cite{tian2008efficient}. We also note that K-Snap lacks theoretical guarantees, as the underlying optimization problem is also NP-hard.


We, therefore, introduce a heuristic algorithm, named \algoName, for the \probName\ problem. \algoName\ effectively meets the size constraint and efficiently produces high-quality summary causal DAGs in practice (as we show in Section \ref{sec:exp}).
Moreover, as we show in Section~\ref{sec:identifiability}, we theoretically guarantee that the summary causal DAG can be used for sound causal inference, which is not possible for graph summarization algorithms in general.




% \vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{1}}) Additional Experiments}}. 
\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{2}})
% \label{rev:point-2}
Improving the presentation}} In response to the reviewers' comments we improved the paper's presentation. The main changes are summarized below:

\noindent
$\bullet$ \textbf{General Improvements.} We enhanced Example \ref{ex:ex1} to clarify what the edges in the graph represent (Section \ref{sec:intro}) and added new examples throughout the paper to provide intuition for key definitions (Examples \ref{ex:causal_DAGs}, \ref{ex:CIs}, and \ref{ex:RB_summary}).
We also elaborated on the necessity of Definition \ref{def:imap} and explained its role in defining the causal DAG summarization problem (Section \ref{sec:sum}).

Additionally, we improved the presentation of the canonical causal DAG (Section~\ref{subsec:canonical_DAG}), clarifying that it is not the objective of our problem; rather, it serves as a tool to formally define causal inference over summary DAGs and guide our algorithm in identifying node contractions that minimize information loss (Section \ref{sec:csep}). We also use the connection between a summary DAG and its corresponding \groundedDAG\ to prove the NP-Hardness of our problem (as explained in Point 1 above). Lastly, we refined Example \ref{ex:canonical_DAG} and Figure \ref{fig:canonical_DAG} to better illustrate how the \groundedDAG\ is defined compared to the original causal DAG and a summary DAG.




\noindent
$\bullet$ \textbf{$d$-separation \& $s$-separation} We added a full definition of $d$-separation (please refer to the revised Section \ref{sec:background}) and improved our explanation on how $s$-separation extends $d$-separation (in the revised Section \ref{sec:ssep}) to address reviewer comments

% \noindent
% \reviewercomment{MR3}{Certain background elements, such as the concept of d-separation and its extension, should be clearly introduced. Definitions that may not directly contribute to the main arguments could be streamlined.}

In particular, $d$-separation is a criterion in a DAG that determines whether two sets of nodes are conditionally independent,
given a third set of nodes. If two sets of nodes $\mb{X}$ and $\mb{Y}$ are $d$-separated by $\mb{Z}$, by definition it means that the paths connecting $\mb{X}$ and $\mb{Y}$ are blocked by nodes form $\mb{Z}$, which makes $\mb{X}$ and $\mb{Y}$ conditionally independent
given $\mb{Z}$.

\emph{$s$-separation} is an extension of $d$-separation, tailored to identify all conditional independence (CI) relations encoded by a summary DAG. $d$-separation can only identify \ci\ using nodes on a causal DAG but is not equipped to identify all \ci\ encoded in a summary DAG, as we illustrate in Example~\ref{ex:without-csep}. 
Intuitively, a summary DAG represents a collection of causal DAGs that are compatible with it, meaning that it could have been obtained from any of those DAGs (similar to \emph{possible worlds} in probabilistic databases \cite{dalvi2007efficient}). Each of these DAGs encodes a different set of \ci. The set of \ci\ encoded by a summary DAG is defined as the intersection of \ci\ that hold in all compatible DAGs.
In this way, using $s$-separation we can ensure we restrict ourselves only to \ci\ that are certainly present in a particular context and can be reliably used for inference. % $s$-separation extends $d$-separation by allowing the identification of valid \ci\ within a summary causal DAG, as opposed to regular causal DAGs.
We also introduce a sound and complete $s$-separation algorithm that leverages the standard $d$-separation algorithm. Please refer to the revised Section \ref{sec:ssep}.



% \vspace{1mm}
\noindent 
\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{3}})  Including an ablation study}} 
In response to the reviewers' request, we included an ablation study in our revised paper (full details are given in Section \ref{subsec:ablation}).

% \noindent
% \reviewercomment{MR4}{Some claims in the paper are not sufficiently supported by experiments. Ablation studies or detailed evaluations of optimization techniques like caching should be conducted to illustrate their efficacy.}

The goal of this study is to assess the effect of our proposed optimizations on the performance of \algoName. To this end, we examine three variants of \algoName\ by disabling each of our main optimizations: (I) No Cache, a version of \algoName\ without caching mechanisms, (ii) No Preprocessing, a version of \algoName\ without the low-cost merge optimization, which contracts low-cost node pairs as a preprocessing step, and (iii) No Optimizations: a variant without either optimization. We did not include the semantic constraint here, as it is not a runtime optimization but rather an extension that restricts permissible contractions.

For quality, we observed that across all baselines, the number of additional edges remained the same despite changes in the number of nodes. This suggests that \emph{our proposed optimizations improve runtime without compromising the algorithm’s quality}. The results indicate that the \emph{caching mechanisms significantly improve runtime (making it run nearly three times faster), while the impact of preprocessing is modest}. For large, dense input causal DAGs, preprocessing can slightly slow down the algorithm. However, it provides noticeable runtime benefits for small, sparse input DAGs (as demonstrated in our experiments; see full results in Section \ref{subsec:ablation}). Therefore, we recommend applying the preprocessing optimization for relatively small (up to 50 nodes), sparse DAGs.

 
 % \vspace{1mm}
\noindent
% {\bf{(\colorbox{pink}{Point \textrm{1}}) Additional Experiments}}. 
\subsubsection*{\bf{(\colorbox{pink}{Point \textrm{4}})  Clarifying our main contributions in relation to prior work.}} We focused our efforts on clarifying our main contributions in relation to prior work:

% \noindent
% \reviewercomment{MR5}{The paper claims novelty but seems to build on existing algorithms with incremental improvements. Clarification on how the proposed method significantly differs from or improves existing approaches is necessary. Including more comprehensive discussions about related work could provide better context.}

% \markos{This answer aims to ``clarify our main contributions'', but we spend 3 paragraphs talking about related work and then one short sentence at the end actually clarifying what \emph{we} did. I would suggest shortening the first two paragraphs here (all of this stuff is in the related work section of the paper anyway) and actually elaborating on the last sentence. The them vs. us ratio should be closer to 50/50}

In our revised paper, we clarified that causal inference is a major theme in recent data management research (please refer to the revised Introduction in Section~\ref{sec:intro}).
Drawing causal conclusions from data fundamentally hinges on
access to background knowledge, which is typically encoded through Causal DAGs. These DAGs are typically created
using domain knowledge or causal discovery methods, both of which are costly, error-prone, and time-consuming. Causal discovery methods also struggle with real-world data and require
significant human intervention for verification. This highlights the need for efficient methods to simplify and verify causal models while preserving essential
information.

Graph summarization is therefore a logical next step. As we mention in the revised Section \ref{sec:related_work}, graph summarization has been extensively studied within the data management community~\cite{bhowmick2022data,fan2012query,liu2014distributed,maneth2016compressing,navlakha2008graph}. 
However, we argue that existing techniques are ill-suited for the \probName\ problem. Graph summarization objectives differ across applications, often prioritizing minimizing the reconstruction error \cite{lee2020ssumm, yong2021efficient}, facilitating accurate query answering \cite{shin2019sweg,maccioni2016scalable}, or enhancing visualizations \cite{jin2017ecoviz,koutra2014vog}. Consequently, existing methods inadequately cater to the objective of preserving causal information, often yielding graphs unsuitable for causal inference. Please refer to Example~\ref{example:example_causal_dag_summary} to explore the implications of this objective mismatch.

We note that our algorithm 
follows a previous line of work ~\cite{tian2008efficient,geisberger2012exact}, where a bottom-up greedy approach is used to identify promising node pairs for contraction. Our main contribution lies in how it estimates merge costs related to the causal interpretation of the graph and the objective of preserving causal information.

Our algorithm aims to simplify high-dimensional causal DAGs
into manageable forms without compromising essential causal information, thereby improving interpretability. Using our technique,
one can summarize an initial causal DAG for simpler verification and
elicitation. Additionally, the summary causal DAG can be directly
used for causal inference. Our approach thereby improves interpretability,
verifiability, and robustness in causal inference, facilitating the adoption of these techniques in data management and various fields of research.


\vspace{4mm}
This concludes the summary of the main revisions in the paper.
Below, you will find detailed responses to the reviewers' comments.

\subsection*{Reviewer \#1}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.W1}} \emph{The paper is more geared towards the AI/machine learning field than data management.} 
% \markos{I think here we are on the right track but there are some missing links. We should say 1. data mgmt people use causality 2. but they often have tons of variables 3. graph summarization could help but is unsuitable for causal graphs 4. so we bring a new technique to enable the data mgmt people to use causality. Currently we skip step 2, and we don't "bring it back to the data mgmt community" when discussing 4. That is, we don't say why summarization \emph{is relevant for causality users from the data management community specifically, as opposed to general causality enthusiasts.}}
\reva{
\textbf{Ans.} As we mention in Point 4 above, causal inference is a major theme in recent data management research~\cite{meliou2010causality, bertossi2017causes, meliou2014causality,salimi2020causal,10.14778/3554821.3554902}. Causality has been incorporated into various data management tasks such as finding the responsibility of inputs toward query answers~\cite{meliou2010causality, meliou2009so, meliou2014causality}, explaining query answers~\cite{salimi2018bias,youngmann2024summarized,youngmann2023explaining,roy2014formal}, data discovery~\cite{galhotra2023metam,youngmann2023causal}, data cleaning~\cite{pirhadi2024otclean,salimi2019interventional}, hypothetical reasoning~\cite{galhotra2022hyper}, and large system diagnostics~\cite{markakis2024sawmill,causalsim,sage, gudmundsdottir2017demonstration}.
However, data management use cases often result in needing high-quality causal models, which are difficult to obtain. % Constructing DAGs through domain knowledge or causal discovery is often costly, error-prone, and time-consuming. Example~\ref{example:example_causal_dag} describes how sensitive graph quality can be to }
% As we see in Example~\ref{example:example_causal_dag},
% Causal inference relies on high-quality causal DAGs, which are often difficult to obtain.
These DAGs are typically created using domain knowledge or causal discovery methods, both of which are costly, error-prone, and time-consuming. 

% Graph summarization is therefore a logical next step. As we mention in the \nameref{sec:related_work} section, graph summarization has also been extensively studied within the data management community~\cite{bhowmick2022data,fan2012query,liu2014distributed,maneth2016compressing,navlakha2008graph}. 
% However, we argue (in \nameref{sec:related_work}) and empirically demonstrate (in Sections \ref{sec:intro} and \ref{sec:exp}) that existing graph summarization techniques are ill-suited for the \probName\ problem.

In this work, we develop a graph summarization technique tailored for causal inference to better support data management and general use cases of causality. Our goal is to simplify high-dimensional causal
DAGs into manageable forms without compromising essential
causal information, thereby improving interpretability. Using our technique, one
can summarize an initial causal DAG (constructed using partial
domain knowledge or causal discovery) for simpler verification and
elicitation. Additionally, the summary causal DAG can be directly
used for causal inference and is more robust to misspecification of
assumptions. Our approach thereby improves interpretability, verifiability, and robustness in causal inference, facilitating the adoption
of these techniques in data management and various fields of research.
}



\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.W2+R1.D2}} \emph{The main graph summary algorithm is heuristics without formal guarantees. // The proposed graph summary algorithm (Algorithms 1 and 2) is based on simple heuristics --- minimizing the number of edges added to the resulting \groundedDAG. However, it does not provide any formal guarantees.} \reva{
\textbf{Ans.} We thank the reviewer for this comment. Indeed, our algorithm does not have theoretical guarantees. As explained now in Section \ref{sec:algorithm} and shown in Theorem \ref{theorem:problem-is-np-hard}, the \probName\ problem is NP-hard and therefore, developing an efficient algorithm with theoretical guarantees is a complex challenge that requires significant effort. 
Consequently, we propose a heuristic algorithm, \algoName, to address the \probName\ problem. As previously mentioned, this algorithm guarantees sound causal inference directly on the summary DAG.
Please refer to Point 1 above for further discussion. 

% \anna{Ideally I'd like to figure out how to hyperlink this just like section numbers or citation numbers, so the reviewers can click to see it... minor point in the grand scheme of things though.}

% Although \algoName\ lacks theoretical guarantees, it effectively satisfies the size constraint and efficiently produces high-quality summary causal DAGs in practice. Specifically, our experiments demonstrated that the resulting summary DAGs are effective for direct causal inference, and that our algorithm produces higher-quality summary DAGs compared to the baselines.  
}


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.W3 + R3.D1}} \emph{There are some small errors in the paper: (a) Line 15 of Algorithm 1 should be outside the for loop.
(b) Last paragraph of page 7: "An invalid pair is a pair of nodes with semantic similarity exceeding the threshold" should be "below" the threshold?
(c) The background on d-separation: $V_{X+1}$ should be $X_{i+1}$?
(d) highly dimensional --> high dimensional.} \reva{
\textbf{Ans.} We thank the reviewers for pointing out these typos. We have carefully proofread the paper to ensure there are no other mistakes. 
} 

% \anna{The mention of \colorbox{pink}{\textbf{R3.D1}} is only in connection with the highly dimensional -> high dimensional comment; I think since we mention \colorbox{pink}{\textbf{R3.D1}} later we don't have to include it here.}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R1.D1}} \emph{Scalable causal inference is an important problem in data science. One school of causal inference is through Causal Directed Acyclic Graphs (DAGs). This paper proposes a simple new algorithm that performs DAG summary. Overall, the paper is well written with theoretical analysis and insights.} \reva{
\textbf{Ans.} We appreciate this feedback. In response to the reviewer’s comments, we have improved the paper's writing for better clarity. Please refer to Point 2 above for more details.
} 

% \anna{Maybe I'm missing something, but how does this relate to Point 2?}




% \vspace{1mm}
% \noindent
% \colorbox{pink}{\textbf{R1.D2}} \emph{The proposed graph summary algorithm (Algorithms 1 and 2) is based on simple heuristics --- minimizing the number of edges added to the resulting canonical causal DAG. However, it does not provide any formal guarantees.} \reva{
% \textbf{Ans.} 
% }


\subsection*{Reviewer \#2}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.W1 + R1.D1}} \emph{The presentation is sometimes very hard to follow. // There are a lot of definitions in the paper, which adds a lot of rigor. However, such presentation also makes it very hard to follow as the readers have to understand every meaning of the definition. I am unsure whether they are all needed to present the problem. It seems that there shall be more intuitive ways to present these definitions as opposed to those with full math notations.} \revb{
\textbf{Ans.} We thank the reviewer for this feedback. In our revised version, we made significant efforts to enhance the paper's readability. This includes revising Examples \ref{ex:ex1} and \ref{ex:canonical_DAG}, clarifying the rationale and necessity of Definition \ref{def:imap}, and explaining the connection between $d$-separation and $s$-separation. Please see Point 2 above for further details. 
}
% \anna{When reading through the paper, I'd like to come back to this point and verify if the intuitive version of a read-through is smooth enough to make this reviewer happy.}


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.W2}} \emph{The novelty is unclear or seems to be limited given the previous works.} \revb{
\textbf{Ans.} Please see Point 4 for a discussion of our main contributions, and refer to the response to R2.D5 for an overview of related methods. 
}


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.W3 + R2.D3}} \emph{Some proofs are missing. // In page 2, the authors claim that they proved the problem of "finding a summary DAG that preserves CI statements to the greatest extent possible, while meeting a node" is NP-hard, yet no proof is given.} \revb{
\textbf{Ans.} As mentioned in Point 1 above, the proof relies on the connection between node contraction and the addition of edges which we establish in Section~\ref{subsec:canonical_DAG}. Thus, in the revised paper we explain the intuition behind this theorem in Section \ref{subsec:canonical_DAG} after presenting the \groundedDAG. We have also refined the proof to improve its readability. The full proof is now provided in \cite{full} due to space limitations.
Please refer to Point 1 above for more details. 


% In more details, Theorem~\ref{theorem:problem-is-np-hard} establishes that finding a summary DAG $(\qg,f)$ whose causal DAG $\cg_{\qg}$ results in the smallest number of added edges $|\edges(\cg_{\qg})|-|\edges(G)|$ is NP-Hard. Specifically, the proof of Theorem~\ref{theorem:problem-is-np-hard} shows that finding a summary DAG $(\qg,f)$ where $|\nodes(\qg)|=k$ and $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$ for some threshold $\tau >0$ is an NP-complete problem. In fact, we prove the stronger claim that finding a summary DAG $(\qg,f)$ where $|\nodes(\qg)|=k$ and 
% \begin{equation}
% \label{eq:specialedges}
%     \left| \set{(X_i,X_j)\in \edges(\cg_{\qg}){\setminus}\edges(G) : f(X_i)=f(X_j} \right|\leq \tau
% \end{equation}
% is NP-hard. If $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$, then~\eqref{eq:specialedges} must hold as well. We establish that finding a summary DAG where~\eqref{eq:specialedges} holds is NP-Hard, and hence finding a summary DAG where $|\edges(\cg_{\qg})|-|\edges(G)|\leq \tau$ is NP-Hard as well. 


% The full proof is now provided in \cite{full} due to space limitations.
}




% \vspace{1mm}
% \noindent
% \colorbox{pink}{\textbf{R2.D1}} \emph{There are a lot of definitions in the paper, which adds a lot of rigor. However, such presentation also makes it very hard to follow as the readers have to understand every meaning of the definition. I am unsure whether they are all needed to present the problem. It seems that there shall be more intuitive ways to present these definitions as opposed to those with full math notations.} \revb{
% \textbf{Ans.} We thank the reviewer for this feedback. In our revised version, we made significant efforts to enhance the paper's readability. This includes revising Examples \ref{ex:ex1} and \ref{ex:canonical_DAG}, clarifying the rationale and necessity of Definition \ref{def:imap}, and explaining the connection between $d$-separation and $s$-separation. Please see Point (2) above for further details.
% }




\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.D2}} \emph{Why Definition 3 is necessary to formally define Problem 1?} \revb{
\textbf{Ans.} Thanks for this comment. This definition is necessary to clarify the purpose of a summary DAG, so we have provided some intuition for its role. Specifically, we now explain in Section \ref{sec:sum} that a valid summary DAG must not imply any conditional independence statement that is not present in the original DAG, although it may omit some independencies that do exist. We call this property an \emph{I-Map}. Additionally, we have revised the problem definition (Problem~\ref{causal-graph-summarization-problem}) to emphasize that a summary DAG must be an I-Map for the probability distribution $\pr$ and maximal for $\pr$. }



% \vspace{1mm}
% \noindent
% \colorbox{pink}{\textbf{R2.D3}} \emph{In page 2, the authors claim that they proved the problem of "finding a summary DAG that preserves CI statements to the greatest extent possible, while meeting a node" is NP-hard, yet no proof is given.} \revb{
% \textbf{Ans.} 
% }


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.D4}} \emph{Section 4.2, it is said that d-separation is an extension of s-separation [70], but it is unclear how it extends the notion because d-separation has not been introduced.} \revb{
\textbf{Ans.} In response to the reviewer’s feedback, we revised Section \ref{sec:background} to formally define $d$-separation. Additionally, in Section \ref{sec:ssep}, we now clarify how $s$-separation extends $d$-separation, enabling the identification of valid conditional independence statements in summary causal DAGs, rather than in standard causal DAGs. We also provide a sound and complete algorithm for $s$-separation, which essentially applies the $d$-separation algorithm to the \groundedDAG\ of the summary DAG. Please also refer to Point 2 above.
}


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.D5}} \emph{ It is said that CaGreS is based on [96], with a new contribution of employing a new greedy policy in estimating the merge cost. The ideas of estimating the merge cost seems to be quite natural and similar greedy idea in selecting contraction nodes has been employed in classic shortest path query algorithms Contraction Hierarchy [1]. It sounds that the novelty is limited.
[1] Exact Routing in Large Road Networks using
Contraction Hierarchies.} 
\revb{ \textbf{Ans.}
Graph summarization is a well-studied problem, as acknowledged in our introduction. In this work, our goal is to study how the problem differs when the graphs in question are causal DAGs.
%
Accordingly, we agree with the reviewer that the meta-algorithm of greedy node contraction via merge cost estimation is a natural idea. What the overview of Section 5 claims as our main contribution is not \emph{that} we estimate merge costs, but \emph{how} we estimate merge costs, to lead to a useful summary graph for our application. 
%
% \anna{I would like to see if we can construct an argument not about the semantics of the application of the problem, but how the metric of shortest path distance in their scenario is distinct from causal information in our case. If we can achieve that, I think I'll feel confident in satisfying this reviewer's concern.}
The provided reference~\cite{geisberger2012exact} interprets directed graphs as \emph{transportation networks}, and as such selects contractions that preserve \emph{shortest path distances} to facilitate \emph{routing queries}. In our case, we interpret them as \emph{causal DAGs}, and as such select contractions that preserve \emph{conditional independence information} to facilitate \emph{accurate causal inference}. The different objective we select means that the method for assigning costs to node merges must be reconsidered from scratch.
%

We have updated the corresponding text in \nameref{sec:related_work} and in Section~\ref{sec:algorithm} for clarity.
}

% \vspace{1mm}
% \noindent
% We include \colorbox{pink}{\textbf{MR6}} below so we address the comment alongside Reviewer 2's remaining comments:

% \noindent
% \reviewercomment{MR6}{
% % \anna{6. 
% Further explanation of how the number of nodes (size constraint for summarization) is selected and justified practically would be beneficial. Also, making clear connections between canonical causal DAGs and the overall summarization problem is necessary for coherence.}% \markos{The first part is addressed in R2.D6, the second part in R2.D7. These are not in this section because only R2 mentons them.} \anna{thank you markos!}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.D6}} \emph{How do users select the number of nodes (size constraint) practically?}
\revb{
\textbf{Ans.} As we now mention in Section \ref{sec:sum}, setting and adjusting a limit on the number of nodes is shown to be relatively straightforward for analysts~\cite{tian2008efficient,DBLP:journals/pvldb/KhanBB17}. We also observe that other summarization problems share similar hyperparameters, including clustering algorithms or $k$-nearest neighbors algorithms~\cite{kramer2013k,likas2003global}.

Nevertheless, we revised the text in Section \ref{sec:conc}, now saying that, as demonstrated in Section \ref{subsec:exp_effectiveness}, the user-defined size constraint may impact the generated summary DAG quality, and users may need to adjust this parameter to obtain a desirable summary. Future research will explore methods to recommend an optimal value for this parameter. For example, a heuristic stopping condition could be added to the algorithm, signaling it to halt if the next merge would result in a significant loss of information.
}



\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R2.D7}} \emph{ In Section 4.1, you define Canonical Causal DAG, but it is quite unclear the usage of such a notion in addressing the overall problem.} \revb{
\textbf{Ans.} We have clarified the use of the \groundedDAG\ in Section \ref{sec:csep}. We note that the \groundedDAG\ is not an objective of our problem; rather, it serves as a tool to formally define causal inference over summary DAGs and to guide our algorithm in identifying node contractions that minimize information loss. We also leverage the connection between summary causal DAG and the \groundedDAG\ to show the hardness of our problem. Please also refer to Point 2 above.}


\subsection*{Reviewer \#3}
\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.W1 + R3.D1}} \emph{ Examples need to come with more explanations, like in Example 1, (1) the meaning of edges should be explained,
otherwise it is hard for non-expert of this domain to understand Figure 1, and (2) what does "highly dimensional" mean? There is no vector or array in Figure 1.} \revc{
\textbf{Ans}. We revised Example~\ref{ex:ex1} to clarify what the edges represent and enhanced Example~\ref{ex:canonical_DAG} to better interpret the concept of the \groundedDAG and its edges. We also corrected the typo; it should have read "high dimensional," referring to the number of attributes in the performance monitoring dataset.
}


\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.W2 + R3.D2}} \emph{ Paper needs a better presentation, like Algorithm 1 and 2 have different code styles, and in Table 2, the dataset name "URLs" has different font from others in the column} \revc{\textbf{Ans.} Thank you for this comment. We revised Algorithm~\ref{algo:cost} and fixed the font issue in Table~\ref{tab:data}. Please also refer to Point 2 above.
} 
% \anna{I'm finding it hard to see where the code styles had differed and how the change addressed this reviewer's concern.}

\vspace{1mm}
\noindent
\colorbox{pink}{\textbf{R3.W3 + R3.D3}} \emph{ Ablation experiments are needed. // The paper highlights that they have several optimizations like caching, but does not provide ablation evaluation on them.
It is better to include experiments to show those optimization techniques do work.} \revc{
\textbf{Ans.} In response to the reviewer's request, we included an ablation study to assess the effectiveness of our two main optimizations. Please refer to the revised Section \ref{subsec:ablation} and Point 3 above.
}

% \vspace{1mm}
% \noindent
% \colorbox{pink}{\textbf{R3.D1}} \emph{ Examples need to come with more explanations, like in Example 1, (1) the meaning of edges should be explained,
% otherwise it is hard for non-expert of this domain to understand Figure 1, and (2) what does "highly dimensional" mean? There is no vector or array in Figure 1.} \revc{
% \textbf{Ans.} 
% }


% \vspace{1mm}
% \noindent
% \colorbox{pink}{\textbf{R3.D2}} \emph{ Paper needs a better presentation, like Algorithm 1 and 2 have different code styles, and in Table 2, the dataset name "URLs" has different font from others in the column.} \revc{
% \textbf{Ans.} 
% }




% \vspace{1mm}
% \noindent
% \colorbox{pink}{\textbf{R3.D3}} \emph{ The paper highlights that they have several optimizations like caching, but does not provide ablation evaluation on them.
% It is better to include experiments to show those optimization techniques do work.} \revc{
% \textbf{Ans.} 
% }

 









==> 03-newFormulation.tex <==





\section{New Formulation}
% \subsection{Semigraphoid-Axioms}
% The semi-graphoid axioms are the following:
% \babak{Having Latex issues with enum...}

% 1.Triviality: $I(A;\emptyset|C)=0$.\\
% 2. Symmetry: $I(A;B|C)=0 \implies I(A;C|B)=0$.\\
% 3. Decomposition: $I(A;BD|C)=0 \implies I(A;B|D)=0$.\\
% 4. Contraction: $I(A;B|C)=0$, $I(A;D|BC)=0 \implies I(A;BD|C)=0$\\
% 5. Weak Union: $I(A;BD|C)=0 \implies I(A;B|CD)=0, I(A;D|BC)=0$	\\
% The semi-graphoid axioms can be summarized using the following identity, which follows from the \e{chain-rule} for mutual information~\cite{Yeung:2008:ITN:1457455}.
% \begin{equation}
% 	\label{eq:chainRule}
% 	I(A;BD|C)=0 \text{ if and only if } I(A;B|C)=0 \text{ and }I(A;D|BC)=0
% \end{equation}

% \subsection{Bayesian Networks}
% \label{sec:BNs}
% Let $G(V,E)$ be a directed Acyclic Graph (DAG), and let $u,v \in V$. We say that $u$ is a \e{parent} of $v$, and $v$ a \e{child} of $u$ if $(u\rightarrow v) \in E$. A \e{directed path} $t=(v_1,v_2,\dots,v_n)$ is a sequence of vertices $(v_1,v_2,\dots,v_n)$ such that there is an edge $(v_i \rightarrow v_{i+1})\in E$ for every $i\in \set{1,\dots,n-1}$. We say that $v$ is a \e{descendant} of $u$, and $u$ an \e{ancestor} of $v$ if there is a directed path from $u$ to $v$.
% A \e{trail} $t=(v_1,v_2,\dots,v_n)$ is a sequence of vertices $(v_1,v_2,\dots,v_n)$ such that there is an edge between $v_i$ and $v_{i+1}$ for every $i\in \set{1,\dots,n-1}$. That is, $(v_i\rightarrow v_{i+1})\in E$ or $(v_i \leftarrow v_{i+1})\in E$ for every $i\in \set{1,\dots,n-1}$. A vertex $v_i$ is said to be \e{head-to-head} with respect to $t$ if $(v_{i-1}\rightarrow v_i)\in E$ and $(v_{i}\leftarrow v_{i+1})\in E$.
% A trail $t=(v_1,v_2,\dots,v_n)$ is \e{active} given $Z\subseteq V$ if (1) every $v_i$ that is a head-to-head vertex with respect to $t$ either belongs to $Z$ or has a descendant in $Z$, and (2) every $v_i$ that is not a head-to-head vertex with respect to $t$ does not belong to $Z$. If a trail $t$ is not active given $Z$, then it is \e{blocked} given $Z$. Let $X,Y,Z\subseteq V$ be pairwise disjoint. We say that $Z$ \e{$d$-separates} $X$ from $Y$ if every trail between $x\in X$ and $y\in Y$ is blocked given $Z$. We denote by $X\bot_{dsep} Y|Z$ that $Z$ $d$-separates $X$ from $Y$


% A Bayesian network encodes the CIs of a probability distribution using a
% DAG. Each node $X_i$ in a Bayesian network corresponds
% to the variable $X_i\in \Omega$, a set of nodes $\alpha$ correspond to the set of variables $X_\alpha$, and $x_i \in \D_i$ is a
% value from the domain of $X_i$. Each node $X_i$ in the network represents the distribution $p(X_i \mid X_{\pi(i)})$ where $X_{\pi(i)}$ is a set of variables that
% correspond to the parent nodes $\pi(i)$ of $i$. The distribution represented by a Bayesian network is
% \begin{equation}\label{eq:BN}
% 	p(x_1,\dots,x_n)=\prod_{i=1}^np(x_i| x_{\pi(i)})
% \end{equation}
% (when $i$ has no parents then $X_{\pi(i)}=\emptyset$).

% Equation~\ref{eq:BN} implicitly encodes a set of $n$ conditional independence statements, called the \e{recursive basis} for the network $G$:
% \begin{equation}
% 	\label{eq:recursiveSet}
% 	\sigmarb(G)\eqdef\set{(X_i; X_1\dots X_{i-1}{\setminus} \pi(X_i) \mid \pi(X_i)): i\in [n]}
% \end{equation}
% Let $\tau\eqdef(A;B|C)$ be a CI where $\tau \notin \sigmarb(G)$.
% The implication problem associated with Bayesian Networks is to determine whether a given CI $\tau$ holds in every probability distribution in which each one of the CIs in $\sigmarb$ holds. In notation, this is denoted $\sigmarb(G) \implies \tau$.
% Let $G(\Omega,E)$ be a DAG generated by the recursive basis $\sigmarb$. That is, the vertices of $G$ are the RVs $\Omega$, and its edges are $E=\set{X_i\rightarrow X_j | X_i\in \pi(X_j)}$.
% Given a CI $\tau=(A;B|C)$, the $d$-separation algorithm efficiently determines whether $C$ $d$-separates $A$ from $B$ in $G$. It has been shown that $\sigmarb \implies \tau$ if and only if $C$ $d$-separates $A$ from $B$ in the DAG $G$ generated by $\sigmarb$~\cite{DBLP:journals/networks/GeigerVP90}.
% \begin{citedtheorem}{\cite{DBLP:journals/networks/GeigerVP90,DBLP:conf/uai/GeigerP88,DBLP:conf/uai/VermaP88}}
% 	\label{thm:soundnessCompletenessdSep}
% 	Let $P(\Omega)$ be a joint probability distribution over the RVs $\Omega$, and $G(\Omega,E)$ be the DAG generated by the recursive basis $\sigmarb(G)$ (see~\eqref{eq:recursiveSet}). Let $\sigmarb^+$ denote the closure of $\sigmarb(G)$ with respect to the semi-graphoid axioms (see~\eqref{eq:chainRule}). The following holds for every three disjoint sets $A,B,C \subseteq \Omega$:
% 	\begin{align*}
% 	\sigmarb(G) \implies (A;B|C) && \text{ iff } && (A;B|C)\in \sigmarb^+ && \text{ iff } && A\bot_{dsep} B|C
% 	\end{align*} 
% \end{citedtheorem}
% Theorem~\ref{thm:soundnessCompletenessdSep} establishes that both the semi-graphoid axioms, and the $d$-separation criterion, are sound and complete for inferring CI statements from the recursive basis. 

% \subsection{Comparing models based on the recursive basis}
% Let $\Omega\eqdef \set{X_1,\dots,X_n}$ be a set of jointly distributed RVs with distribution $P$. We denote by $\mathcal{G}(P)$ the set of DAGs that are an I-Map for $P$. Formally:
% \begin{align*}
% 	\mathcal{G}(P)\eqdef \set{\text{DAGs }G\text{ s.t. }\sigmarb(G) \text{ holds in }P}
% \end{align*}
% Let $G_1(\Omega,E_1)$ and $G_2(\Omega,E_2)$ denote two DAGs that are I-Maps for  $P$ (i.e., $G_1,G_2\in 	\mathcal{G}(P)$).
% We say that $G_2$ is superior to $G_1$, in notation $G_2 \succ G_1$, if for every $\sigma\in \sigmarb(G_1)$, it holds that  $\sigmarb(G_2) \implies \sigma$.
% We observe that $\succ$ such defined does not necessarily constitute a complete order. We say that $G(\Omega,E)$ is \e{maximal for $P$} if $G$ is an I-Map for $P$ (i.e., $G\in \mathcal{G}(P)$), and there does not exist any $G'\in \mathcal{G}(P)$ such that $G'\succ G$. 
% In this work, we are given a DAG $G$ that is a minimal I-Map of a joint distribution $P$. Our goal is to efficiently return all $k$-summaries that are maximal for $P$. \babak{ Is this the goal ??}
% \begin{example}
% 	Consider the causal DAG $G_1$ in Figure~\ref{fig:g1}. Figure~\ref{fig:qg} presents the graph $H_1$ which is a $4$-summary of $G_1$. In particular, $\sigmarb(H_1)=\set{(D;A|BC), (E;ABC|D)}$. Clearly, $\sigmarb(H_1)\subset \sigmarb(G_1)$, and hence $H_1$ is an I-Map for $P$, and $H_1\in 	\mathcal{G}(P)$. Figure~\ref{fig:example} presents $H_2$, which is also a $4$-summary of $G_1$. In this case $\sigmarb(H_2)=\set{(E;AC|BD)}$. Now, observe that from the semi-graphoid axioms (see~\eqref{eq:chainRule}), it holds that $I(E;ABC|D)=0 \implies I(E;AC|BD)=0$. Therefore, by definition, we have that $H_1\succ H_2$. Hence, $H_2$ will not be returned by our algorithm.
% \end{example}

% \begin{figure}
% 	\centering
% 	\includegraphics[scale = 0.6]{figures/DAG summary example.pdf}
% 	\caption{DAG $H_2$, which is a $4$-summary of of the DAG in Figure~\ref{fig:g1}. Note that $\sigmarb(H_2)=\set{(E;AC|BD)}$\label{fig:example}} 
% \end{figure}

% \subsection{Contracting Vertices in DAGs}
% In this short section, we prove a simple lemma that characterizes node contractions that maintain acyclicity in DAGs.
% \begin{lemma}
% 	\label{lem:contractDAG}
% Let $G(V,E)$ be a DAG, and let $A,B\in V$. Let $H$ denote the graph that results from $G$ by contracting $A$ and $B$. Then $H$ contains a cycle if and only if $G$ contains a directed path $P$ from $A$ to $B$ (or $B$ to $A$), where $|P|\geq 2$.
% \end{lemma}
% \begin{proof}
% 	Let $P$ be a directed path from $A$ to $B$, such that $|P|\geq 2$. Let $X$ be $A$'s successor in $P$, and $Y$ be $B$'s predecessor in $P$. By our assumption that $|P|\geq 2$, $X\notin \set{A,B}$, but $Y$ may be the same as $X$. Now, consider the graph $H$. By definition, $H$ contains a node $AB$, with an incoming edge from $Y$, and an outgoing edge to $X$. If $X=Y$, we immediately get the cycle $AB\rightarrow X \rightarrow AB$. Otherwise, we consider the subpath $P'$ (of $P$) from $X$ to $Y$ ($X\underset{P'}{\rightsquigarrow} Y$) in $G$. This results in the following cycle in $H$: $Y\rightarrow AB \rightarrow X\underset{P'}{\rightsquigarrow} Y$.
	
% 	Now, suppose that $H$ contains the cycle $C$. $C$ must contain the node $AB$. Otherwise, the cycle is included in $G$, which leads to a contradiction that $G$ is a DAG. Let $Y$ and $X$ be the incoming and outgoing vertices, respectively, to $AB$ in $C$. Then, there is a directed path $P$ from $X$ to $Y$ in $H$ that avoids $AB$. That is, every vertex and edge on the path $P$ belongs to $G$ as well. Hence, $P$ is a directed path from $X$ to $Y$ in $G$. Since $Y$ is incoming to $AB$, then $Y$ is incoming to either $A$ or $B$ in $G$. Assume, wlog, that $Y\rightarrow A \in E$. Since $X$ is an outgoing vertex from $AB$, then it is outgoing from from either $A$ or $B$ (or both). If $X$ is outgoing from $A$, then we get the following cycle in $G$: $Y\rightarrow A \rightarrow X \underset{P}{\rightsquigarrow}Y$. Since $G$ is a DAG, this brings us to a contradiction.
% 	Therefore, $X$ must be outgoing from $B$ and not $A$.  But this gives us the following directed path from $B$ to $A$: $$A\leftarrow Y \underset{P}{\leftsquigarrow} X \leftarrow B.$$ This completes the proof.
% \end{proof}


\subsection{Vertex-Contraction as Addition of Edges}
\label{sec:contractionAsEdgeAddition}
% Let $S$ and $T$ denote two sets of CIs over the variable-set $\set{X_1,\dots,X_n}$.
% We say that $S\implies T$ if $S \implies \sigma$ for every CI $\sigma \in T$. We say that $S$ and $T$ are equivalent, in notation $S\equiv T$, if $S\implies T$ and $T \implies S$.
% For a DAG $G$, and a vertex $v\in \nodes(G)$, we denote by $\child_G(v)\eqdef\set{x\in \nodes(G): (v,x)\in \edges(G)}$ the child-nodes of $v$ in $G$, by $\desc_G(v)$, the descendants of $v$, which are the vertices $y\in \nodes(G)$ for which there is a directed path from $v$ to $y$ (we assume that $v\in \desc_G(v)$), and by $\nondesc_G(v)\eqdef \nodes(G){\setminus}\desc_G(v)$ the vertices of $G$ that are not descendants of $v$ in $G$. For a set of vertices $S\subseteq \nodes(G)$, we let $\desc_G(S)\eqdef \bigcup_{u\in S}\desc_G(u)$, and by $\nondesc_G(S)\eqdef \bigcap_{u\in S}\nondesc_G(u)$. In particular, if $S=\set{u,v}$, then $\nondesc_G(uv)\eqdef \nondesc_G(u)\cap \nondesc_G(v)$.

% In what follows, we let $u,v\in \nodes(G)$ where $u$ precedes $v$ in the topological order of $\nodes(G)$, and that meet the conditions of Lemma~\ref{lem:contractDAG}. We let $H$ be the DAG that results from contracting $u$ and $v$, and we let $X_{uv}\in \nodes(H)$ the vertex that results from contracting $u$ and $v$. We denote by $G'$ the DAG where $\nodes(G')=\nodes(G)$, and 
% \begin{align*}
% 	\edges(G')\eqdef \edges(G)&\cup \set{(x,y): x\in \pi_G(u)\cup \pi_G(v), y\in \set{u,v}} \\
% 	&\cup \set{(x,y): x\in \set{u,v}, y\in \child_G(u)\cup \child_G(v)} \\
% 	&\cup \set{(u,v)}
% \end{align*}
% We prove some simple lemmas that will be useful later on.
% \begin{lemma}
% 	The following holds:
% 	\begin{align}
% 		&\pi_{H}(X_{uv})=\pi_{G'}(u)&& \pi_{G'}(v)=\pi_{G'}(u){\cup} \set{u}  \label{eq:lem:contractionAddedges1:1}\\
% 		&\child_H(X_{uv})=\child_{G'}(v) && \child_{G'}(u)=\child_{G'}(v){\cup} \set{v} \label{eq:lem:contractionAddedges1:2}\\
% 	%	&\desc_{H}(X_{uv}){\setminus}\set{X_{uv}}=\desc_{G'}(v){\setminus}\set{v} && \desc_{G'}(u)= \desc_{G'}(v){\cup} \set{v}\\
% 		&\nondesc_H(X_{uv})=\nondesc_{G'}(u) && \nondesc_{G'}(v)=\nondesc_{G'}(u){\cup} \set{u} \label{eq:lem:contractionAddedges1:4}
% 	\end{align}
% \end{lemma}
% \begin{proof}
% By the definition of $G'$, it holds that $\pi_{G'}(u)=\pi_G(u)\cup \pi_G(v)$. Since $(u,v)\in \edges(G')$, then $\pi_{G'}(v)=\pi_{G'}(u) \cup \set{u}$.
% Similarly, $\child_{G'}(v)=\child_G(u)\cup \child_G(v)$, and since $(u,v)\in \edges(G')$, then $\child_{G'}(u)=\child_{G'}(v) \cup \set{v}$.
% By definition of edge contraction, it holds that $\pi_H(X_{uv})=\pi_G(u)\cup \pi_G(v)=\pi_{G'}(u)$, proving~\eqref{eq:lem:contractionAddedges1:1}.
% Also, by definition of edge contraction, it holds that $\child_H(X_{uv})=\child_G(u)\cup \child_G(v)=\child_{G'}(v)$, proving~\eqref{eq:lem:contractionAddedges1:2}.

% We now prove~\eqref{eq:lem:contractionAddedges1:4}. Let $t\in \nondesc_H(X_{uv})$. If $t \notin \nondesc_{G'}(u)$, then $t\in \desc_{G'}(u){\setminus}\set{v}$. This means that there is a directed path $P$ from $u$ to $t$ in $G'$. Let $s$ be the first vertex on this path (after $u$). Since $s\in \child_{G'}(u){\setminus}\set{v}$, then by the definition of $G'$, $s\in \child_G(u)\cup \child_G(v)$. By the definition of edge contraction, $s\in \child_H(X_{uv})$. Since $s\notin uv \cup \pi_G(u)\cup \pi_G(v)$, then every directed path starting at $s$ in $G$ remains a directed path in $H$. But this means that there is a directed path from $X_{uv}$ to $t$ (via $s$); contradicting the assumption that $t\in \nondesc_H(X_{uv})$. 
% Now, let $t\in \nondesc_{G'}(u)$. If $t\notin \nondesc_H(X_{uv})$, then $t\in \desc_H(X_{uv}){\setminus}\set{X_{uv}}$.  This means that there is a directed path $P$ from $X_{uv}$ to $t$ in $H$. Let $s$ be the first vertex on this path (after $X_{uv}$). Since $s\in \child_{H}(X_{uv})$, then by the definition of $H$, $s\in \child_G(u)\cup \child_G(v)$. But then, by the definition of $G'$, it holds that $s\in \child_{G'}(u)$. Since no edges are removed by the transition from $G$ to $G'$, there is a directed path from $u$ to (via $s$) in $G'$; contradicting the assumption that $t\in \nondesc_{G'}(u)$. 
% \end{proof}
% \begin{lemma}
% 	\label{lem:contractionAddedges2}
% 	Let $t\in \nodes(G)$ such that $t\notin \set{u,v}\cup \child_G(u)\cup \child_G(v)$. Then it holds that:
% 	\begin{align}
% 		& \pi_{G'}(t)=\pi_H(t) \text{ and } \label{eq:sameParents}\\
% 		&\nondesc_{G'}(t){\setminus}uv=\nondesc_{H}(t){\setminus}\set{X_{uv}} \text{ and }\label{eq:tNotChild} \\
% 		& \set{u,v}\subseteq \nondesc_{G'}(t)  \text{ if and only if }  X_{uv}\in \nondesc_{H}(t) \label{eq:uvXuvparent} 
% 	\end{align}
% 	Now, let  $t\in \nodes(G)$ such that $t\notin \set{u,v}\cup \pi_G(u)\cup \pi_G(v)$. Then:
% 	\begin{align}
% 		&\child_{G'}(t)=\child_H(t) \text{ and }  \label{eq:sameChildren}\\
% 		& \desc_{G'}(t){\setminus}uv=\desc_{H}(t){\setminus}\set{X_{uv}} \label{eq:tNotParent}\\
% 		& \set{u,v}\subseteq \desc_{G'}(t)  \text{ if and only if }  X_{uv}\in \desc_{H}(t)
% 	\end{align}
% \end{lemma}
% \begin{proof}
% By the definition of contraction, the only vertices in $G$ whose parent-set can potentially change following the contraction of $u$ and $v$ belong to the set $uv \cup \child_G(u) \cup \child_G(v)$.
% By the definition of $\edges(G')$, the only vertices in $G$ whose parent-set can potentially change belong to the set $uv \cup \child_G(u) \cup \child_G(v)$.
% Therefore, if $t\notin uv \cup \child_G(u) \cup \child_G(v)$, then $\pi_{G'}(t)=\pi_{H}(t)=\pi_G(t)$. This proves~\eqref{eq:sameParents}.

% By the definition of contraction, the only vertices in $G$ whose child-set can potentially change following the contraction of $u$ and $v$ belong to the set $uv \cup \pi_G(u) \cup \pi_G(v)$.
% By the definition of $\edges(G')$, the only vertices in $G$ whose child-set can potentially change belong to the set $uv \cup  \pi_G(u) \cup \pi_G(v)$.
% Therefore, if $t\notin uv \cup \pi_G(u) \cup \pi_G(v)$, then $\child_{G'}(t)=\child_{H}(t)=\child_G(t)$. This proves~\eqref{eq:sameChildren}.

% We now prove~\eqref{eq:tNotChild};
% Let $s\in \nondesc_{H}(t){\setminus}\set{X_{uv}}$. If $s\notin \nondesc_{G'}(t)$, then $s\in \desc_{G'}(t)$. That is, there is a directed path $P$ from $t$ to $s$ in $G'$. Let us assume wlog that $P$ is the shortest directed path from $t$ to $s$ in $G'$. By this assumption, exactly one of the following holds: (1) $u,v \notin \nodes(P)$ (2) $u\in \nodes(P)$, $v\notin nodes(P)$ (3) $v\in \nodes(P)$, $u\notin nodes(P)$, or (4) $(u,v)\in \edges(P)$.
% In the first case, every edge of $P$ is also an edge of $\edges(G)$, that does not enter or exit $\set{u,v}$. Therefore, $P$ is a directed path in $H$, a contradiction. In case (2), since $\pi_{G'}(u)=\pi_H(X_{uv})$ (see~\eqref{eq:lem:contractionAddedges1:1}), and $\child_{G'}(u)=\child_H(X_{uv}){\setminus}\set{v}$ (see~\eqref{eq:lem:contractionAddedges1:2}), then the path with nodes $X_{uv}\cup(\nodes(P)\setminus\set{u}) $, is a directed path in $H$ from $s$ to $t$; a contradiction.
% In case (3), since $\child_{G'}(v)=\child_H(X_{uv})$ (see~\eqref{eq:lem:contractionAddedges1:2}), and $\pi_{G'}(v)=\pi_H(X_{uv}){\setminus}\set{u}$ (see~\eqref{eq:lem:contractionAddedges1:1}), then the path with nodes $X_{uv}\cup(\nodes(P)\setminus\set{v}) $, is a directed path in $H$ from $s$ to $t$; a contradiction. Finally, if $(u,v)\in \edges(P)$, then since $\pi_{G'}(u)=\pi_H(X_{uv})$ and $\child_{G'}(v)=\child_H(X_{uv})$, then the path with nodes $X_{uv}\cup (\nodes(P){\setminus}uv)$, is a directed path from $s$ to $t$ in $H$; a contradiction.
% For the other direction, let $s\in \nondesc_{G'}(t){\setminus} uv$. If $s\notin \nondesc_H(t)$, then there is a directed path $P$ from $t$ to $s$ in $H$. If $X_{uv}\notin \nodes(P)$, then $\edges(P)\subseteq \edges(G)\subseteq \edges(G')$, and hence $P$ is a directed path from $t$ to $s$ in $G'$. Otherwise, if $X_{uv}\in \nodes(P)$, then since $\pi_H(X_{uv})=\pi_{G'}(u)$, $\child_H(X_{uv})=\child_{G'}(v)$, and $(u,v)\in \edges(G')$, then replacing $X_{uv}$, with the edge $(u,v)$ results in a directed $t,s$-path in $G'$; a contradiction.
% \eat{
% If $u,v \notin \nodes(P)$, then $P$ is a path in $H$, and hence $s\in \desc_H(t)$, which leads to a contradiction. If $u\in \nodes(P)$, then since $(u,v)\in \edges(G')$, and $\child_{G'}(u)=\child_{G'}(v)\cup \set{v}$, then $P$ can be made to go through both $u$ and $v$, and we can assume that $u,v \in \nodes(P)$. Likewise,  if $v\in \nodes(P)$, then since $(u,v)\in \edges(G')$, and $\pi_{G'}(u)\cup\set{u}=\pi_{G'}(v)$, then $P$ can be made to go through both $u$ and $v$, and we can assume that $u,v \in \nodes(P)$. So, we assume that $uv \subseteq \nodes(P)$. Since $H$ is a DAG, then by Lemma~\ref{lem:contractDAG}, there is no directed path between $u$ and $v$ whose length is greater than 2. But this means that $(u,v)\in \edges(P)$. But this means that $\nodes(P){\setminus}uv \cup X_{uv}$ form a directed path in $H$, contradicting the assumption that $s\in \nondesc_{H}(t)$. 
% }
% \end{proof}
% \begin{theorem}
% 	\label{thm:contractionEdgeAddition}
% Let $G$ be a DAG, $u,v \in \nodes(G)$ where we assume wlog that $u$ precedes $v$ in the topological order of $\nodes(G)$. Let $H$ be the DAG that results from contracting $u$ and $v$. Then $\Sigma_{\text{RB}}(H)\equiv \Sigma_{\text{RB}}(G')$.
% \end{theorem}
% \begin{proof}
% 	We first prove that $\Sigma_{\text{RB}}(G')\implies \Sigma_{\text{RB}}(H)$. We divide to cases.
% 	Let $(X_i; B_i|\pi_H(X_i))\in \Sigma_{\text{RB}}(H)$, where $X_{uv}\notin B_i\cup \pi_H(X_i)\cup \set{X_i}$.
% 	In particular, $X_i\in \nodes(G)$, and $X_i\notin \set{u,v}\cup \child_H(X_{uv})=\set{u,v}\cup \child_G(u)\cup \child_G(v)$.
% 	By~\eqref{eq:tNotChild}, we have that $\pi_{G'}(X_i)=\pi_H(X_i)$, and that $\nondesc_{G'}(X_i){\setminus}uv=\nondesc_{H}(X_i){\setminus}X_{uv}$.
% 	Therefore, we have that $(X_i;\nondesc_{H}(X_i){\setminus}\set{X_{uv}}|\pi_{G'}(X_i))_{G'}$. Since
% 	 $B_i\subseteq \nondesc_{H}(X_i){\setminus}\set{X_{uv}}$, then, by decomposition, we have that $\Sigma_{\text{RB}}(G')\implies (X_i; B_i| \pi_H(X_i))$.
	 
% 	Now, let $(X_i; X_{uv}B_i|\pi_H(X_i))\in \Sigma_{\text{RB}}(H)$. In this case as well $X_i\in \nodes(G)$, and $X_i\notin \set{u,v}\cup \child_H(X_{uv})=\set{u,v}\cup \child_G(u)\cup \child_G(v)$. By~\eqref{eq:tNotChild}, we have that $\pi_{G'}(X_i)=\pi_H(X_i)$, and that $\nondesc_{G'}(X_i){\setminus}uv=\nondesc_{H}(X_i){\setminus}X_{uv}$. 
% 	By , we have that $X_{uv}\in \nondesc_{H}(X_i)$ iff $uv \subseteq \nondesc_{G'}(X_i)$. Therefore, $B_iX_{uv}\subseteq \nondesc_{H}(X_i)$ iff $B_iuv\subseteq \nondesc_{G'}(X_i)$. This means that $\Sigma_{\text{RB}}(G')\implies (X_i;\nondesc_{G'}(X_i)|\pi_{G'}(X_i))$. By decomposition, we have that $\Sigma_{\text{RB}}(G')\implies (X_i;B_iuv|\pi_{H}(X_i))$ as required.


% 	Now, suppose that $X_{uv}\in \pi_H(X_i)$, or that $X_i \in \child_H(X_{uv})$. Since $X_i\in \nodes(G){\setminus}\set{u,v}$, then by~\eqref{eq:lem:contractionAddedges1:2}, we have that $X_i\in \child_{G'}(v){\setminus}\set{v}$. Therefore, $\pi_{G'}(X_i)=\pi_H(X_i){\setminus}\set{X_{uv}}\cup \set{u,v}$. 
% 	By~\eqref{eq:tNotChild}, we have that:
% 	\begin{align*}
% 		\nondesc_{G'}(X_i){\setminus}\pi_{G'}(X_i)&=\nondesc_{G'}(X_i){\setminus}(\pi_H(X_i){\setminus}\set{X_{uv}}\cup uv)\\
% 		&=(\nondesc_{G'}(X_i){\setminus}uv){\setminus}(\pi_H(X_i){\setminus}\set{X_{uv}})\\
% 		&\underbrace{=}_{\eqref{eq:tNotChild}}(\nondesc_{H}(X_i){\setminus}\set{X_{uv}}){\setminus}(\pi_H(X_i){\setminus}\set{X_{uv}}) \\
% 		&=\nondesc_{H}(X_i){\setminus}\pi_H(X_i)
% 	\end{align*} 
% Therefore, $\Sigma_{\text{RB}}(G')\implies (X_i; \nondesc_H(X_i){\setminus}\pi_H(X_i) \mid \pi_H(X_i){\setminus}\set{X_{uv}}\cup \set{u,v})$. 
% Finally, we consider the case where $X_i=X_{uv}$. By construction of $G'$, and by~\eqref{eq:lem:contractionAddedges1:4}, it holds that:
% \begin{align}
% 	\Sigma_{\text{RB}}(G')&\implies (u; \nondesc_{G'}(u){\setminus}\pi_{G'}(u) \mid \pi_{G'}(u)) \label{eq:GImpliesHContractionAxiom:1}\\
% 	\Sigma_{\text{RB}}(G')&\implies (v; \nondesc_{G'}(u){\setminus}\pi_{G'}(u) \mid \pi_{G'}(u)\cup \set{u}) \label{eq:GImpliesHContractionAxiom:2}
% \end{align}
% By applying the contraction axiom on~\eqref{eq:GImpliesHContractionAxiom:1} and~\eqref{eq:GImpliesHContractionAxiom:2}, we get that 
% $$\Sigma_{\text{RB}}(G') \implies (uv; \nondesc_{G'}(u){\setminus}\pi_{G'}(u) \mid \pi_{G'}(u)).$$
% Using the fact that hat $\pi_H(X_{uv})=\pi_{G'}(u)$ (see~\eqref{eq:lem:contractionAddedges1:1}), and that $\nondesc_H(X_{uv})=\nondesc_{G'}(u)$ (see~\eqref{eq:lem:contractionAddedges1:4}), we get that 
% $$\Sigma_{\text{RB}}(G') \implies (uv; \nondesc_{H}(X_{uv}){\setminus}\pi_{H}(X_{uv}) \mid\pi_{H}(X_{uv})).$$
% Since $B_i \subseteq \nondesc_{H}(X_{uv}){\setminus}(\pi_{H}(X_{uv})\cup \set{X_{uv}})$, this proves the claim.


% Now, for the other direction. Let $(X_i;B_i \mid \pi_{G'}(X_i))\in \Sigma_{\text{RB}}(G')$. If $u,v \notin X_i\cup B_i \cup \pi_{G'}(X_i))$, then $X_i\notin \set{u,v}\cup \child_G(u) \cup \child_G(v)$. By~\eqref{eq:tNotChild}, it holds that $\pi_H(X_i)=\pi_{G'}(X_i)$, and that $\nondesc_{G'}(X_i){\setminus}uv=\nondesc_H(X_i){\setminus}X_{uv}$. Since $B_i\subseteq \nondesc_{G'}(X_i){\setminus}uv=\nondesc_H(X_i){\setminus}X_{uv}$, then  $\Sigma_{\text{RB}}(H)\implies (X_i;B_i \mid \pi_{G'}(X_i))$.

% If $uv \subseteq B_i$, then $u,v\notin \pi_{G'}(X_i)$, then $X_i\notin uv\cup \child_G(u)\cup \child_G(v)$. By~\eqref{eq:tNotChild}, we have that $\pi_H(X_i)=\pi_{G'}(X_i)$, and that $\nondesc_{H}(X_i){\setminus}X_{uv}=\nondesc_{G'}(X_i){\setminus}uv$. Therefore, $B_i{\setminus}uv\subseteq \nondesc_{H}(X_i)$, and by~\eqref{eq:uvXuvparent}, if $uv \subseteq B_i \subseteq \nondesc_{G'}(X_i)$, then $X_{uv}\in \nondesc_{H}(X_i)$.
% Therefore, $\Sigma_{\text{RB}}(H)\implies (X_i;B_i{\setminus}uv \cup X_{uv} \mid \pi_{G'}(X_i))$, and since $X_{uv}=uv$, then $\Sigma_{\text{RB}}(H)\implies (X_i;B_i \mid \pi_{G'}(X_i))$. 

% Since $(u,v)\in \edges(G')$, we are left with two other cases. 
% First, that $(u;B_u \mid \pi_{G'}(u))$, and second $(v; B_v \mid \pi_{G'}(v))$. 
% By $d$-separation in $H$, the following holds:
% \begin{align}
% \Sigma_{\text{RB}}(H) & \implies (X_{uv}; \nondesc_H(X_{uv}){\setminus}\pi_H(X_{uv}) \mid \pi_H(X_{uv})) \nonumber \\
% & \underbrace{\implies}_{\eqref{eq:lem:contractionAddedges1:1},~\eqref{eq:lem:contractionAddedges1:4}}(X_{uv}; \nondesc_{G'}(u){\setminus}\pi_{G'}(u) \mid \pi_{G'}(u)) \nonumber \\
% & \implies (uv ; \nondesc_{G'}(u){\setminus}\pi_{G'}(u) \mid \pi_{G'}(u)) \label{eq:HImpliesG1}
% \end{align}

% By~\eqref{eq:lem:contractionAddedges1:1}, it holds that $\pi_{G'}(v)= \pi_{G'}(u)\cup \set{u}$. 
% By~\eqref{eq:lem:contractionAddedges1:4}, it holds that 
% \begin{align*}
% B_v \subseteq \nondesc_{G'}(v){\setminus}\pi_{G'}(v)&=(\nondesc_{G'}(u)\cup \set{u}){\setminus}(\pi_{G'}(u)\cup \set{u})\\
% &=\nondesc_{G'}(u){\setminus}\pi_{G'}(u)
% \end{align*}
% Therefore, $B_v \cup B_u \subseteq \nondesc_{G'}(u){\setminus}\pi_{G'}(u)$.
% In other words, by~\eqref{eq:HImpliesG1}, we have that;
% \begin{align*}
% &\Sigma_{\text{RB}}(H) \implies (uv ; B_u \cup B_v \mid \pi_{G'}(u))  \text{ if and only if } \\
% &\Sigma_{\text{RB}}(H) \implies (u ; B_u \cup B_v \mid \pi_{G'}(u)) ,  (v ; B_u \cup B_v \mid \pi_{G'}(u)\cup \set{u}) 
% \end{align*}
% Since  $\pi_{G'}(v)= \pi_{G'}(u)\cup \set{u}$, then
% overall, we have that $\Sigma_{\text{RB}}(H) \implies (u;B_u \mid \pi_{G'}(u))$, and $\Sigma_{\text{RB}}(H) \implies (v;B_v \mid \pi_{G'}(v))$. This completes the proof.
% \end{proof}

% Let $G$ be an ADMG (Acyclic Directed Mixed Graph) representing a causal BN. Let $G'$ be an ADMG where $\nodes(G')=\nodes(G)$. We say that $G'$ is a supergraph of $G$ if $\edges(G)\subseteq \edges(G')$. In this case we also say that $G$ is \e{compatible} with $G'$.
% \begin{definition}[Summary DAG for CBN]
% 	\label{def:summaryDAG}
% 	A summary-DAG of an ADMG $G$ is a pair $(H,f)$, where $H$ is an ADMG with nodes $\nodes(H)$, edges $\edges(H)$, and $f$ is a function that partitions the vertices $\nodes(H)$ among the vertices $\nodes(H)$, such that:
% 	\begin{enumerate}
% 		\item For every $v\in \nodes(G)$, there exists exactly one node $u_v\in \nodes(H)$ such that $v\in f(u_v)$.
% 		\item If $(u,v)\in \edges(G)$, then $f(u)=f(v)$ or $(f(u),f(v))\in \edges(H)$.
% 	\end{enumerate}
% \end{definition}
% \begin{definition}[Compatible with summary-DAG]
% 	Let $(H,f)$ be a pair where $H$ is an ADMG. A DAG $G$ is \e{compatible} with $H$ if $H$ is a summary-DAG for $G$.
% \end{definition}

% \begin{definition}[Grounded-DAG]
% 	\label{def:groundedDAG}
% 	Let $(H,f)$ be a summary-DAG for an ADMG $G$. Let $\langle X_1,\dots,X_n \rangle$ denote a complete topological order over $\nodes(G)$. We define that grounded-DAG associated with $(H,f)$, denoted $G_H$ as follows: $\nodes(G_H)=\nodes(G)$, and
% 	\begin{align*}
% 		(X_i,X_j)\in \edges(G_H) &\text{ if and only if }&  (X_i,X_j)\in \edges(G) \\
% 		&\text{ or }& (f(X_i),f(X_j))\in \edges(H) \\
% 		&\text{ or }& f(X_i)=f(X_j) \text{ and }i<j
% 	\end{align*}
% \end{definition}

% We observe that, by definition, $G_H$ is compatible with the summary-DAG $(H,f)$.
	

\begin{theorem}[Soundness and Completeness of $d$-separation in supergraphs]
	\label{thm:dSep}
	In an ADMG $G'$, let $X,Y,Z\subseteq \nodes(G')$ be disjoint sets of variables. If $X$ and $Y$ are $d$-separated by $Z$ in $G'$, then in any ADMG $G$ compatible with $G'$, $X$ and $Y$ are $d$-separated by $Z$ in $G$. That is:
	\begin{align}
		(X;Y|Z)_{G'} \implies (X;Y|Z)_{G}
	\end{align}
	If $X$ and $Y$ are $d$-connected by $Z$ in $G'$, then there exists a compatible ADMG $G$, compatible with $G'$, where $X$ and $Y$ are $d$-connected by $Z$ in $G$.
\end{theorem}
\begin{proof}
	Suppose that $X$ and $Y$ are $d$-separated by $Z$ in $G'$ (i.e., $(X;Y|Z)_{G'}$). If $X$ and $Y$ are $d$-connected by $Z$ in $G$, then let $P$ denote the unblocked path between $X$ and $Y$, relative to $Z$. Since $\edges(G')\supseteq \edges(G)$, then clearly $P$ is a path in $G'$ as well. Consider any triple $(x,w,y)$ on this path. If this triple has one of the forms $$\set{x\rightarrow w\rightarrow y, x\leftarrow w\leftarrow y, x \leftrightarrow w \rightarrow y, x\leftarrow w \leftrightarrow y},$$ then since $P$ is unblocked in $G$, relative to $Z$, then $w\notin Z$. Since $w\notin Z$, then the subpath $(x,w,y)$ is also unblocked in $G'$.
	If the triple has one of the forms:
	$$\set{x\leftrightarrow w\leftarrow y, x\rightarrow w\leftrightarrow y, x\rightarrow w \leftarrow y},$$
	then since $P$ is unblocked in $G$, relative to $Z$, then $\desc_G(w) \cap Z\neq \emptyset$. Since $\edges(G')\supseteq \edges(G)$, then $\desc_G(w)\subseteq \desc_{G'}(w)$. Therefore, $\desc_{G'}(w) \cap Z\neq \emptyset$. Consequently, we have, again, that the subpath $(x,w,y)$ is unblocked in $G'$.
	Overall, we get that every triple $(x,w,y)$ on the path $P$ is unblocked in $G'$, relative to $Z$, and hence $X$ and $Y$ are $d$-connected in $G'$, a contradiction.
	
	By definition, $G'$ is compatible with $G'$. Therefore, if $X$ and $Y$ are $d$-connected by $Z$ in $G'$, then by the completeness of $d$-separation, there exists a probability distribution that factorizes according to $G'$ in which the CI $(X;Y|Z)$ does not hold. This proves completeness.
\end{proof}

Let $(H,f)$ denote a summary-DAG, and let $X\subseteq \nodes(H)$. We denote by $f(X)\eqdef \bigcup_{x\in X}f(x)$.
\begin{corollary}[Soundness and Completeness of $d$-separation in Cluster-DAGs]
		In a summary-DAG $(H,f)$, let $X,Y,Z\subseteq \nodes(H)$ be disjoint sets of vertices. If $X$ and $Y$ are $d$-separated by $Z$ in $H$, then in any ADMG $G$ compatible with $H$, $f(X)$ and $f(Y)$ are $d$-separated by $f(Z)$ in $G$. That is:
	\begin{align}
		(X;Y|Z)_{H} \implies (f(X);f(Y)|f(Z))_{G}
	\end{align}
	If $X$ and $Y$ are $d$-connected by $Z$ in $H$, then there exists an ADMG $G$, compatible with $H$, where $f(X)$ and $f(Y)$ are $d$-connected by $f(Z)$ in $G$.
\end{corollary}
\begin{proof}
	Let $G_H$ denote the grounded DAG corresponding to $H$. By Theorem~\ref{thm:contractionEdgeAddition}, $\Sigma_{\text{RB}}(H)\equiv \Sigma_{\text{RB}}(G_H)$. Since $\edges(G)\subseteq \edges(G_H)$, the claim follows from Theorem~\ref{thm:dSep}.
\end{proof}

\subsection{Do-Calculus in Summary DAGs}
We now make the assumption that $G$ is a causal Bayesian network (CBN) whose underlying graph is an Acyclic Directed Mixed Graph (ADMG). That is, the rules of do-calculus hold for $G$. Let $H$ be a summary-DAG for $G$ with grounded-DAG $G_H$. In this section, we show that the rules of Do-calculus are sound and complete in the summary-DAG $H$. This was already proved in~\cite{anand2022effect}. We provide  simpler proof that relies on the equivalence $\Sigma_{\text{RB}}(G)\equiv \Sigma_{\text{RB}}(G_H)$ proved in Theorem~\ref{thm:contractionEdgeAddition}, and the soundness and completeness of $d$-separation in $G_H$ (Theorem~\ref{thm:dSep}). This result is not surprising because $G_H$ is a causal BN where $\edges(G) \subseteq \edges(G_H)$. Pearl already observed in~\ref{pearl2009causality} that "In general, the addition of arcs to a causal diagram can impede, but never assist, the identification of causal effects in nonparametric models. This is because such addition reduces the set of d-separation conditions carried by the diagram; hence, if causal effect derivation fails in the original diagram, it is bound to fail in the augmented diagram".


Fo a subset of vertices $X\subseteq \nodes(G)$, we let $G_{\overline{X}}$ denote the graph that results from $G$ by removing all incoming edges to the vertices $X$, by $G_{\underline{X}}$ the graph that results from $G$ by removing all outgoing edges from the vertices $X$. For a subset of vertices $X\subseteq \nodes(G){\setminus}X$, we denote by $G_{\overline{X}\underline{Z}}$ the graph that results from $G$ by removing all incoming edges into $X$ and all outgoing edges from $Z$.

\begin{lemma}
	\label{lem:mutilatedGraphInclusion}
Let $G$ be ADMG, and let $G'$ be an ADMG where $\nodes(G')=\nodes(G)$, and $\edges(G')\supseteq \edges(G)$. Let $A,B,C\subseteq \nodes(G)$ be disjoint sets of variables, and let $X,Z \subseteq \nodes(G)$. Then:
\begin{align}
	(A;B|C)_{G'_{\overline{X}\underline{Z}}} \implies (A;B|C)_{G_{\overline{X}\underline{Z}}} 
\end{align}
\end{lemma}
\begin{proof}
	We show that $\edges(G_{\overline{X}\underline{Z}})\subseteq \edges(G'_{\overline{X}\underline{Z}})$, and the claim then follows from Theorem~\ref{thm:dSep}.
	Let $(u,v)\in \edges(G_{\overline{X}\underline{Z}})\subseteq \edges(G) \subseteq \edges(G')$. By definition, $u\notin Z$ and $v \notin X$. But this means that $(u,v)\in \edges(G'_{\overline{X}\underline{Z}})$, which completes the proof.
\end{proof}

\begin{corollary}
	\label{corr:mutilatedSummaryDAG}
	Let $G$ be ADMG, and let $(H,f)$ be a summary-DAG for $G$. 
    Let $A,B,C\subseteq \nodes(H)$ be disjoint sets of nodes, and let $X,Z \subseteq \nodes(H)$. Then:
	\begin{align}
		(A;B|C)_{H_{\overline{X}\underline{Z}}} \implies ({\bf A};{\bf B}|{\bf C})_{G_{\overline{{\bX}}\underline{{\bZ}}}} 
	\end{align}
where for $U \subseteq \nodes(H)$, we denote ${\bf U}\eqdef f(U)$. 
\end{corollary}
\begin{proof}
Let $G_{H_{\overline{X}\underline{Z}}}$ denote the grounded DAG corresponding to $H_{\overline{X}\underline{Z}}$. By Theorem~\ref{thm:contractionEdgeAddition}, $\Sigma_{\text{RB}}(H_{\overline{X}\underline{Z}})\equiv \Sigma_{\text{RB}}(G_{H_{\overline{\bX}\underline{\bZ}})}$, and hence $(A;B|C)_{H_{\overline{X}\underline{Z}}}$ if and only if $({\bf A};{\bf B}|{\bf C})_{G_{H_{{\overline{{\bf X}}\underline{{\bf Z}}}}}}$. Since $\edges(G_H)\supseteq \edges(G)$, then by Lemma~\ref{lem:mutilatedGraphInclusion}, it holds that if $({\bf A};{\bf B}|{\bf C})_{G_{H_{{\overline{{\bf X}}\underline{{\bf Z}}}}}}$, then $({\bf A};{\bf B}|{\bf C})_{G_{{\overline{{\bf X}}\underline{{\bf Z}}}}}$. Overall, we have that:
\begin{align}
	(A;B|C)_{H_{\overline{X}\underline{Z}}} \Leftrightarrow ({\bf A};{\bf B}|{\bf C})_{G_{H_{{\overline{{\bX}}\underline{{\bZ}}}}}} \implies ({\bf A};{\bf B}|{\bf C})_{G_{\overline{{\bX}}\underline{{\bZ}}}} 
\end{align}
which proves the claim.
\end{proof}

\begin{theorem}[Soundness of Do-Calculus in supergraphs]
Let $G$ be a causal BN (CBN) encoding an interventional distributions $P(\cdot \mid do(\cdot))$. Let $G'$ be an ADMG where $\edges(G)\subseteq \edges(G')$. For any disjoint subsets $X,Y,Z,W \subseteq \nodes(G)$, the following three rules hold:%

{\footnotesize
\begin{align*}
	{\bf R}_1: && (Y;Z|X,W)_{G'_{\overline{X}}} &\implies P(Y\mid do(X),Z,W)=P(Y\mid do(X),W) \\
	{\bf R}_2: && (Y;Z|X,W)_{G'_{\overline{X}\underline{Z}}} &\implies P(Y\mid do(X),do(Z),W)=P(Y\mid do(X),Z, W) \\
	{\bf R}_3: && (Y;Z|X,W)_{G'_{\overline{X}\overline{Z(W)}}} &\implies P(Y\mid do(X),do(Z),W)=P(Y\mid do(X), W) 
\end{align*}}%
where $Z(W)$ is the set of vertices in $Z$ that are not ancestors of any vertex in $W$. That is, $Z(W)=Z{\setminus}\ancs_{G'}(W)$ where $\ancs_{G'}(W)\eqdef \bigcup_{w\in W}\ancs_{G'}(w)$.
\end{theorem}
\begin{proof}
	If $(Y;Z|X,W)_{G'_{\overline{X}}}$, then by Lemma~\ref{lem:mutilatedGraphInclusion}, it holds that $(Y;Z|X,W)_{G_{\overline{X}}}$. By the soundness of do-calculus for causal BNs, we get that $P(\bY \mid do(\bX),\bZ,\bW)=P(\bY\mid do(\bX),\bW) $. 
	If $ (Y;Z|X,W)_{G'_{\overline{X}\underline{Z}}}$, then by Lemma~\ref{lem:mutilatedGraphInclusion}, it holds that $ (Y;Z|X,W)_{G_{\overline{X}\underline{Z}}} $. By the soundness of do-calculus for causal BNs, we get that $P(Y\mid do(X),do(Z),W)=P(Y\mid do(X),Z, W) $. 
	Finally, if $(Y;Z|X,W)_{G'_{\overline{X}\overline{Z(W)}}}$, then by Lemma~\ref{lem:mutilatedGraphInclusion}, it holds that $(Y;Z|X,W)_{G_{\overline{X}\overline{Z(W)}}}$. By the soundness of do-calculus for causal BNs, we get that $P(Y\mid do(X),do(Z),W)=P(Y\mid do(X), W) $. 
\end{proof}


\begin{theorem}[Soundness of Do-Calculus in summary-DAGs]
	Let $G$ be a causal BN (CBN) encoding an interventional distributions $P(\cdot \mid do(\cdot))$, that is compatible with the summary-DAG $(H,f)$. For any disjoint subsets $X,Y,Z,W \subseteq \nodes(H)$, the following three rules hold:%
	
	{	\footnotesize
	\begin{align*}
		{\bf R}_1: && (Y;Z|X,W)_{H_{\overline{X}}} &\implies  P(\bY \mid do(\bX),\bZ,\bW)=P(\bY\mid do(\bX),\bW)   \\
		{\bf R}_2: && (Y;Z|X,W)_{H_{\overline{X}\underline{Z}}} &\implies P(\bY\mid do(\bX),do(\bZ),w)=P(\bY\mid do(\bX),\bZ, \bW) \\
		{\bf R}_3: && (Y;Z|X,W)_{H_{\overline{X}\overline{Z(W)}}} &\implies P(\bY \mid do(\bX),do(\bZ),\bW)=P(\bY\mid do(\bX), \bW)
	\end{align*}
}%
where, $\bU\eqdef(U)$ for every $U\in \nodes(H)$, and $Z(W)$ is the set of vertices in $Z$ that are not ancestors of any vertex in $W$. That is, $Z(W)=Z{\setminus}\ancs_H(W)$ where $\ancs_H(W)\eqdef \bigcup_{w\in W}\ancs_H(w)$.
\end{theorem}
\begin{proof}
	If $(Y;Z|X,W)_{H_{\overline{X}}} $, then by Corollary~\ref{corr:mutilatedSummaryDAG}, it holds that $(\bY;\bZ|\bX,\bW)_{G_{\overline{X}}}$. By the soundness of do-calculus for causal BNs, we get that $P(\bY \mid do(\bX),\bZ,\bW)=P(\bY\mid do(\bX),\bW)$.
	If $(Y;Z|X,W)_{H_{\overline{X}\underline{Z}}}$,  then by Corollary~\ref{corr:mutilatedSummaryDAG}, it holds that $(\bY;\bZ|\bX,\bW)_{G_{\overline{X}\underline{Z}}}$. By the soundness of do-calculus for causal BNs, we get that $P(\bY\mid do(\bX),do(\bZ),w)=P(\bY\mid do(\bX),\bZ, \bW)$.
	Finally, if $(Y;Z|X,W)_{H_{\overline{X}\overline{Z(W)}}}$, then by Corollary~\ref{corr:mutilatedSummaryDAG}, it holds that $(\bY;\bZ|\bX,\bW)_{G_{\overline{X}\underline{Z(W)}}}$. By the soundness of do-calculus for causal BNs, we get that $P(\bY \mid do(\bX),do(\bZ),\bW)=P(\bY\mid do(\bX), \bW) $.
\end{proof}

\begin{theorem}[Completeness of Do-Calculus in summary-DAGs]
	Let $(H,f)$ be an ADMG that is a summary-DAG for $G$, and let $X,Y,W,Z \subseteq \nodes(H)$ be disjoint sets of variables. If $Y$ is $d$-connected to $Z$ in $H_{\overline{X}}$ with respect to $X\cup W$, then there exists an ADMG $G'$ compatible with $H$, such that $f(Y)$ is $d$-connected to $f(Z)$ in $G'_{\overline{f(X)}}$ with respect to $f(X\cup W)$.
\end{theorem}
\begin{proof}
	Consider $G_H$, the grounded-DAG of $(H,f)$, that is, by definition, compatible with $H$.
	If $Y$ is $d$-connected to $Z$ in $H_{\overline{X}}$ with respect to $X\cup W$, then by Definition~\ref{def:groundedDAG}, it holds that $y$ is $d$-connected to $z$ in $G_{H_{\overline{f(X)}}}$ with respect to $f(X\cup W)$, for every $y\in f(Y)$ and $z\in f(Z)$. 
	Therefore,  $f(Y)$ is $d$-connected to $f(Z)$ in $G_{H_{\overline{f(X)}}}$ with respect to $f(X\cup W)$.
\end{proof}

==> CI_eval.tex <==
\subsection{Evaluating The Objective}
\label{subsec:ci_eval}

% As discussed in Section \ref{subsec:ci_counting},
Evaluating causal graph summarization algorithms naively and exactly is computationally infeasible, so in Section \ref{subsec:ci_counting}, we introduced both lower and estimated upper bounds
% as a means
to % approximately conduct our evaluation.
conduct a best-case evaluation
given realistic computing constraints.
Here, before proceeding with the performance evaluation, we investigate how these estimations compare with the true number of CIs.

In this minor foray,
we randomly generated
1295
quotient causal DAGs with up to $13$ nodes and calculated the true size of the CI statements they encode, and estimations with a $30$-second timeout.
% These causal DAGs are all guaranteed to have conditional independence statements, as we prohibited the consideration of complete graphs.
% Be aware that the following findings may have some selection bias due to this timeout threshold.

% is it valid to only approximate the singletons? yes
First, we ask: "Is it a valid means to approximate the size of the overall size of CI statements set by only counting conditional independence statements between singletons (except for the conditioning set)?" 
As illustrated in Figure \ref{fig:singletons}, our answer is yes. We found that, in practice, there is a strong correspondence between the graph's entire CI set size and the subset containing only singleton statements.
Understanding what causes these subtle differences may be a fruitful question to develop in future work.

\begin{figure}
\centering
\includegraphics[scale = 0.33]{writing/figures/true_vs_singleton.pdf}
\caption{The size of the overall CI set \emph{can} be captured by the subset concerning singletons.}
\label{fig:singletons}
\end{figure}

From a bird's-eye view, the lower and upper bounds seem very promising in Figure \ref{fig:aggregate_comparison}; of course, the aggregation may portray a smaller skew than actuality on a per-estimation basis, so we also analyzed how each estimation compared to the true value to better understand the skew.

\begin{figure}
\centering
\includegraphics[scale = 0.33]{writing/figures/overall_singleton.pdf}
\caption{Aggregate lower bound \& upper bound accuracy}
\label{fig:aggregate_comparison}
\end{figure}

% is the lower bound sound and how far is it? yes
% \anna{talk about the histograms}
As illustrated in Figure \ref{fig:lower_bound_comparison},
% "Is the lower bound sound? How tight of a bound is it?"
the lower bound is sound in practice and
is exactly the right value 16.6\% of the time. However,
20.6\%
of the lower bound estimations were $0$. In these cases, all CI statements in the quotient graph were lost in the moralization step. This would mean that in such graphs, the entire CI set captures independencies that happen along paths of colliders.
% 1295 - 354 - 344 = 597
% 597 / 1295 = 46.1\% but not right
% 1295 - 215 - 267 = 813
% 813 / 1295
Beyond the two extremes,
it remains the case that the remaining 62.8\% of the estimations are roughly % evenly
uniformly
distributed between 0-100\% below the true size of the CI set.
While this lower bound is theoretically sound, the lower bound estimations are often (at least 20\% of the time) not sufficiently informative to determine promising causal graph summarizations.

\begin{figure}
\centering
\includegraphics[scale = 0.33]{writing/figures/lb_vs_singleton.pdf}
\caption{Comparing the lower bound estimation with the true size of the CI set of singleton statements.}
\label{fig:lower_bound_comparison}
\end{figure}

% is the upper bound complete and how far is it? no
% perhaps i should try the stupid no-cut upper bound for size maybe
While the upper bound is not theoretically sound or complete, our results in Figure \ref{fig:upper_bound_comparison} seem to indicate this estimation is
% 505 / 1295
exactly correct 39\% of the time
% 141 up to 10% below
% 58 up to 10% above
% 505 + 141 + 58 = 704
% 704 / 1295 = 54.4%
% another 56 up to 20% above
% another 160 down to 20% below
% 704 + 56 + 160 = 920
% 920 / 1295 = 71.0%
and within 20\% of the true value 71\% of the time.
Furthermore, 
% 267 bottom estimations of 0
% 212 of them have an exact upper bound estimation
79.4\% of the lower-bound estimations of 0 have an exact upper bound estimation,
% 215 correct lower bound estimations
% 212 wrong lower bound but correct upper bound estimation
% 215 + 212 = 427
% 427 / 1295 = 33%
% By introducing the guideline that a lower-bound estimation of 0 means we should
giving us a guideline of having an exact estimation 1/3 of the time, roughly twice that of having only the lower bound.

\begin{figure}
\centering
\includegraphics[scale = 0.33]{writing/figures/ub_vs_singleton.pdf}
\caption{Comparing the upper bound estimation with the true singleton CI set size}
\label{fig:upper_bound_comparison}
\end{figure}

% how often does it work properly as a comparator between two graphs differently summarized?
% if i were to draw a chart that says, across many summarizations of the same node size we can see a clear pattern
Lastly, we endeavored to evaluate these estimations as a comparator.
% prototype
% predict tie if upper bounds are equal
% true positives 19
% false positives 4
% false negatives 2
% true negatives 408
% precision (false positives) 83%
% recall (false negatives) 90%
% predict win if upper bound is higher
% ub1 > ub2 and 1 won (true positive) 151
% ub1 > ub2 and 1 did not win (false positive) 8
% 1 won but ub didn't compare (false negative) 5
% ub1 < ub2 and 2 won (true positive) 247
% ub1 < ub2 and 2 did not win (false positive) 4
% 2 won but ub didn't compare (false negative) 9
% true negatives 433 - everything above = 9
% true positives 151 + 247 = 398
% false positives 8 + 4 = 12
% false negatives 5 + 9 = 14
% precision 97.1%
% recall 96.6%
% overall we get:
% true positives 398 + 19 = 417
% false positives 12 + 4 = 16
% false negatives 14 + 2 = 16
% precision / recall are both 96.3%
To do this, we generated
% actual
% true positive ties 22
% false positive ties 4
% false negative ties 5
% true positive g1 219
% false positive g1 16
% false negative g1 13
% true positive g2 312
% false positive g2 13
% false negative g2 15
% true positive total: 22 + 219 + 312 = 553
% false positive total: 4 + 16 + 13 = 33
% false negative total: 5 + 13 + 15 = 33
% 94.4% precision and recall
573 % 433
% recounting
% true positive comparison 518 + 22 = 540
% false positive comparison = 33
% false negative comparison = 33
graphs with up to 10 nodes, randomly created two different quotient graphs from each, and ran both brute force counting and estimations to identify whether the estimations are effective in determining which graph preserved more CI statements. Again, we used a timeout of $30$ seconds for each estimation. We found that simply using the upper bound estimation as the metric of comparison resulted in precision and recall of
94.2\% % 96.3\%
compared to brute force.
% \anna{describe the dependency with the size of the graph and the min cut assumption}
As seen in Figure \ref{fig:upper_bound_comparison}, we see a decrease in accuracy as the size of the quotient causal DAGs gets bigger, likely due to the assumption that having a single minimum cut represent how two nodes are separated is less true as the quotient DAG gets larger.
% \anna{how to illustrate / diagram the results? probably just a table and then the line graph}

\begin{figure}
\centering
\includegraphics[scale = 0.33]{writing/figures/qg_size_vs_pr.pdf}
\caption{The desired size of the quotient DAG impacts the quality of our estimation metric comparator}
\label{fig:upper_bound_comparison}
\end{figure}


% \paragraph*{CI counting evaluations}
% \brit{present an experiment on small synthetic dags where you can count the real number of CIs compared with the approximation method. you should add a graph where the x-axis is the number of nodes in the graph (the number of edges should be fixed to something like $|V|^2-constant\_number$) and the y-axis is the num of CIs. you should have three lines for the lower bound, real number and upper bound}

==> algorithms2.tex <==
\section{The CAMBA Algorithm}
\label{sec:algorithm}
\brit{the properties of the algorithm - subset of cis, causal directionality}
The \probName\ problem has been proven to be NP-hard, as illustrated in Theorem \ref{problem-is-np-hard}.
% In response, we have developed an % highly \anna{i'm kind of embarrassed to say something like that...}
% efficient algorithm to find a quotient causal DAG for an input causal DAG.
While our algorithm, called \algoName, lacks theoretical guarantees, % \anna{for... runtime? it does guarantee foundational things like that the graph is acyclic and such},
it is advantageous in that it satisfies the constraints of \probName\ and, in practice, is able to find high-quality quotient causal DAGs efficiently, even for large input DAGs.

Our \algoName\ algorithm employs the following optimizations:
\begin{itemize}
    \item A greedy approach to identify promising candidate node pairs for merging.
    \item A method for obtaining an initial approximation of the CI set, which may be prohibitively large.
    \item Inexpensive update method to maintain a set of \ci.
    \item A top-down partitioning approach to identify sufficiently small subgraphs for the Greedy procedure to handle.
 
\end{itemize}
% We conclude this section by examining the time complexity and limitations of our \algoName\ algorithm.
To begin, we discuss the limitations of a naive brute-force algorithm. We then gradually introduce our optimizations, and finally describe the full \algoName\ algorithm (Section \ref{subsec:camba}). 
To simplify the presentation, we assume in this section that there is no semantic constraint, meaning that every node merge is possible. However, to support a semantic constraint, the algorithm checks whether each merge violates the semantic constraint before proceeding with it.

\paragraph{\bf Brute Force}  
A naive brute force algorithm explores all possible quotient causal DAGs with up to $k$ nodes; for each candidate, it enumerates the recoverable \ci\ through $C$-separation.
This algorithm finds the optimal solution to the \probName\ problem, but runs in exponential time, % $e^{O(n)}$ \brit{Anna, what are e and n?},
due to the exponential number of partitions to explore and the exponential number of \ci\ to be enumerated for each quotient causal DAG. As we show next, our proposed \algoName\ algorithm overcomes these limitations by avoiding iterating over every possible partition of the nodes and enumerating CI statements only for small subgraphs. 


\subsection{Greedy Search}
\label{subsec:greedy}

Next, we introduce our Greedy Search procedure, which will be utilized as a subroutine on subgraphs in our \algoName\ algorithm.

This procedure is given in Algorithm \ref{algo:greedy_search}. It employs an iterative, bottom-up strategy to merge nodes, gradually reducing their number until the desired size is reached (lines 3-11).
During each iteration, the algorithm selects the node pair that, upon merging, preserves the highest number of \ci (lines 9-11).
This approach improves upon the exhaustive search by reducing the space of potential partitions explored during the search. By selecting a pair of nodes to merge at each iteration, we narrow the partition search space to only those partitions that place both nodes within the same cluster. 

The algorithm employs two further optimizations: (1) it uses the Markov boundary (the set of a given node's parents, children, and shared parents of its children, more in Section \ref{subsec:markov-boundary-partitioning}) to approximate the input causal DAG \ci\ set. Intuitively, we improve the initial \ci\ set initialization in the first step of Greedy Search by using CI statements derived from each nodes' Markov boundary (the \textsc{FindCIsCSep} procedure, line~2); (2) The algorithm updates the \ci\ set in linear time with respect to the input \ci\ set after each node contraction, to avoid repeatedly generating the \ci\ set from scratch (the \textsc{UpdateCISet} procedure, line~8).

\setlength{\textfloatsep}{2px}
\SetInd{1.0ex}{1.0ex}
\begin{algorithm}[t]
\small
	\DontPrintSemicolon
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{A quotient causal DAG $\qg$ and a number $k$. }
	\Output{A quotient causal DAG $\mathcal{G}_{\text{output}}$ with $k$ nodes.} \BlankLine
  \SetKwFunction{FindCIsCSep}{\textsc{FindCIsCSep}}
  \SetKwFunction{Merge}{\textsc{Merge}}
   \SetKwFunction{HasCycle}{\textsc{HasCycle}}
    \SetKwFunction{UpdateCISet}{\textsc{UpdateCISet}}

	
 $\mathcal{G}_{\text{output}}  \gets \qg$\\

 $\mathcal{CI} \gets \FindCIsCSep(\qg)$ \\
   \While{ $|\mathcal{G}_{\text{output}} |>k$ }
   {
   \For{$(\boldsymbol{U}, \boldsymbol{V}) \in \mathcal{G}_{\text{output}}.\text{nodes}$}
   {
    $\mathcal{G}_{UV} \gets \mathcal{G}_{\text{output}}\Merge(\boldsymbol{U}, \boldsymbol{V})$\\
    \If{$\mathcal{G}_{UV}.$\HasCycle()}{
    continue\\
    }
    updated\_CI$\gets \UpdateCISet(\mathcal{CI},\boldsymbol{U}, \boldsymbol{V} ,\qg)$\\
    \If{$|\mathcal{CI}| < |\text{updated\_CI}|$}{
    $\mathcal{CI} \gets \text{updated\_CI}$\\
    $\qg \gets \mathcal{G}_{UV}$
    }
   }
  

  }
  \Return $\mathcal{G}_{\text{output}}$

\caption{Greedy Search}\label{algo:greedy_search}
\end{algorithm} 

\paragraph{\bf \ci\ Set Approximation}
We improve our \ci\ initialization in our Greedy Search algorithm by enumerating two CI statements 
from each node as a seed: one relating the node to the rest of the graph via its Markov boundary and one relating the node to its indirect ancestors via its direct parents.
This takes the naive $O(e^n)$ enumeration of all CI statements out of the \ci\ initialization step and replaces it with a polynomial-time initialization. This procedure is depicted in Algorithm \ref{algo:graph_to_graphoid}.

To illustrate, consider the causal DAG in Figure \ref{fig:causal_dag}. For the node of \verb|airport traffic|, this algorithm will emit one conditional independence statement separating it from
all other nodes in the graph given its Markov boundary, namely \verb|airport|, \verb|population density|, and \verb|departure delay|.
% \verb|departure state| and \verb|departure city|, its indirect ancestors, when conditioned on \verb|airport| and \verb|population density|, its direct parents.
The algorithm will also emit a second conditional independence statement separating \verb|airport traffic| from
% all other nodes in the graph given its Markov boundary, namely \verb|airport|, \verb|population density|, and \verb|departure delay|.
\verb|departure state| and \verb|departure city|, its indirect ancestors, when conditioned on \verb|airport| and \verb|population density|, its direct parents.
% \brit{Anna add an intuitive description of the algo}
% \anna{TODO: include an example based on, say, the figure 1 graph}
% \anna{for each node we will emit two CI statements: node sep rest of graph given MB, and node sep rest of ancestors given parents, so i'll take an example node from the figure two graph, say, D, and emit D indep A given BC and D indep A given BCE}
In order to avoid repeatedly determining sets of ancestors for each node, we optimize retrieval of each node's second conditional independence statement by iteratively removing the leaves from the graph; after all, the Markov boundary of a node without children is solely the set of its direct parents.

\setlength{\textfloatsep}{2px}
\SetInd{1.0ex}{1.0ex}
\begin{algorithm}[t]
\scriptsize
	\DontPrintSemicolon
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{A causal DAG $\cg$. }
	\Output{A set of CIs $\mathcal{CI}$.} \BlankLine
  \SetKwFunction{GetMBCIs}{\textsc{GetMBCIs}}
   \SetKwFunction{FindCIsCSep}{\textsc{FindCIsCSep}}
 

  $\mathcal{CI} \gets \emptyset$\\
\While{$|\cg.nodes| > 0$}
{
$\mathcal{CI}.add(\GetMBCIs(\mathcal{G}))$\\
leaves $\gets$ nodes in $\mathcal{G}$ with no outbound edges\\
$\mathcal{G}.remove($leaves)\\
}
\Return \FindCIsCSep($\mathcal{CI}$)\\
 
\caption{Faster CI Set Initialization}\label{algo:graph_to_graphoid}
\end{algorithm}

\paragraph{\bf Fast \ci\ Set Update}
Our second optimization involves avoiding the need to regenerate the CI set from scratch after each merge. Instead, we update the CI set in linear time with respect to the input CI set within our Greedy Search (line 8 in Algorithm \ref{algo:greedy_search}). This is achieved by utilizing the fact that node contraction is a sound transformation for preserving \ci\ (as shown in Proposition \ref{prop:node_contraction}). Therefore, using $C$-separation, we can focus on determining which \ci\ would be lost when performing a node contraction operation.

Algorithm \ref{algo:fast_update} depicts our subroutine for efficiently updating a \ci\ set after a node contraction. 
It describes Boolean conditions which determine the subsequent behavior of the subroutine, illustrated in Table \ref{table:update_conditions}.
The notation $[U]$ refers to some set of nodes that contains $U$ (namely, $U \in [U]$). $\mb X$, $\mb Y$, and $\mb Z$ are the sets in the considered CI statement ($\mb X \indep_{C} \mb Y $ | $\mb Z$), and $U, V$ are the nodes to be merged.





\setlength{\textfloatsep}{2px}
\SetInd{1.0ex}{1.0ex}
\begin{algorithm}[t]
\scriptsize
	\DontPrintSemicolon
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{A \ci\ set $\mathcal{CI}$, a pair of nodes $(\boldsymbol{V}, \boldsymbol{U})$, and a quotient causal DAG $\qg$. }
	\Output{An updated \ci\ set $\mathcal{CI}^{n}$.} \BlankLine
  \SetKwFunction{RemoveCondition}{\textsc{RemoveCondition}}
  \SetKwFunction{KeepCondition}{\textsc{KeepCondition}}
\SetKwFunction{SecondPassCondition}{\textsc{SecondPassCondition}}
\SetKwFunction{CheckGraphCondition}{\textsc{CheckGraphCondition}}
\SetKwFunction{SecondPassKeepCondition}{\textsc{SecondPassKeepCondition}}



  
	% \SetKwFunction{Moralize}{\textsc{Moralize}}
 % \SetKwFunction{FindMinCut}{\textsc{FindMinCut}}
	
 $\mathcal{CI}^{n} \gets \emptyset$\\
  second\_pass\_set$ \gets \emptyset$\\
 
   \For{ $CI \in \mathcal{CI}$ }
   {
  

   
   \If{$\RemoveCondition(CI, \boldsymbol{V}, \boldsymbol{U})$}{
    continue\\
    }
    \If{$\KeepCondition(CI, \boldsymbol{V}, \boldsymbol{U})$}{
    $\mathcal{CI}^{n}.add(CI)$\\
   }
    \If{$\SecondPassCondition(CI, \boldsymbol{V}, \boldsymbol{U})$}{
     second\_pass\_set$.add(CI)$\\
   }

    \If{$\CheckGraphCondition(CI, \boldsymbol{V}, \boldsymbol{U})$}{
     second\_pass\_set$.add(CI)$\\
     $(\boldsymbol{X}, \boldsymbol{Y}, \boldsymbol{Z}) \gets CI$\\
     $\boldsymbol{Z}' \gets \boldsymbol{Z}$
     but replace $\boldsymbol{U},\boldsymbol{V}$ with the merged $\boldsymbol{UV}$\\
     \If{$\qg.d\_seperated(\boldsymbol{X}, \boldsymbol{Y}, \boldsymbol{Z}')$}{
        $\mathcal{CI}^{n}.add(CI)$\\
     }
   }
   }
     \For{ $CI \in $second\_pass\_set }
   {
     \If{$\SecondPassKeepCondition(CI, \boldsymbol{V}, \boldsymbol{U})$}{
    $\mathcal{CI}^{n}.add(CI)$\\
   }
  }
  \Return $\mathcal{CI}^{n}$

 
\caption{Update \ci\ Set Subroutine}\label{algo:fast_update}
\end{algorithm} 




\begin{table}[]
    \centering
    \small
    \begin{tabular}{ |p{40mm}| p{40mm}| }
    \hline
        Condition & Qualifying CI Statements (output \verb|TRUE| if holds) \\
        \hline\hline
        \textsc{RemoveCondition} & $[U] \indep [V] | Z$ \\
        \hline
        \textsc{KeepCondition} & $[UV] \indep Y | Z$ \\
        \hline
        \textsc{SecondPassCondition} & $[U] \indep Y | Z$ \\
        & or $[U] \indep Y | [V]$ \\
        & or $X \indep Y | [U]$ \\
        \hline
        \textsc{CheckGraphCondition} & $X \indep Y | Z$ where $U, V \notin X \cup Y \cup Z$ \\
        & or $X \indep Y | [UV]$ \\
        \hline
        \textsc{SecondPassKeepCondition} & $[U] \indep Y | Z$ if $[UV] \indep Y | Z$ \\
        & $[U] \indep Y | [V]$ if $[UV] \indep Y | Z$ \\
        & $X \indep Y | [U]$ if $[UV] \indep Y | Z$ \\
        \hline
    \end{tabular}
    \caption{Conditions used in the Update \ci\ Set Subroutine (Algorithm \ref{algo:fast_update})}
    \label{table:update_conditions}
\end{table}

\vspace{3mm}
The Greedy Search algorithm unblocks the exponential time bottlenecks of the Brute Force algorithm, as we no longer need to iterate over every possible partitioning of the nodes or generate the set of \ci. However, as this algorithm is polynomial with respect to the size of the (approximated) \ci\ set of the input graph, it may still not be fast enough for our task. In what comes next, we describe our efforts to overcome this challenge.




 

\subsection{Top-Down Markov Boundary Partitioning}
\label{subsec:markov-boundary-partitioning}

To overcome the exponential scale of the input DAG's CI set, we propose a top-down partitioning approach to identify sufficiently small subgraphs for the Greedy Search to handle. 

To preserve as many \ci\ as possible, we have developed a top-down method that seeks to greedily identify bisections of the input causal DAG that will retain the highest number of \ci. The key factor in this algorithm is its guiding metric, which determines which of the exponentially many cuts should be chosen to preserve the most \ci.
One approach to finding our metric-maximizing split is to identify a single representative CI statement that implies the most CI relationships. By partitioning the graph according to this "densest" representative statement, we can ensure that all $C$-separation CI statements that cross the partition will be retained in the resulting quotient causal DAG.

We identify such representative CI statements
by identifying the \emph{Markov boundary}~\cite{pearl1988probabilistic} of each node in the graph.
The Markov boundary of a node $V$, denoted as $MB(V)$, includes its parents, children, and the other parents of all of its children. It is the minimal set of nodes required to separate $V$ from the rest of the nodes in $\cg$. Each node $V$ and its Markov boundary $MB(V)$ can produce the following CI statement:
$$V \indep \mathcal{V}{\setminus}\{V\}{\setminus}MB(V) | MB(V)$$

As depicted in Algorithm \ref{algo:mb_algo}, we operate a priority queue in which subgraphs of the input graph $\cg$ are prioritized for splitting based on size and semantic similarity; we initialize the queue with $\cg$ itself (line 2) and continue to prioritize large subgraphs with low semantic similarity. For each subgraph we obtain from the priority queue, we enumerate a Markov boundary for each node (line 8) in search of the "densest" representative statement in the subgraph.
% \brit{ANNA, please add an intuitive description of how this algorithm operates.}
Since this partitioning algorithm does not guarantee acyclicity out-of-the-box, we randomly perturb the partition borders until we meet our acyclicity goal (lines 13-22).
% \anna{we have a priority queue, prioritized based on size and semantic similarity so we split groups that are large and low similarity. for each item we take out, we enumerate a markov boundary for each node}
If no partitions are found through the Markov boundary search, a simple acyclic partition is taken via topological ordering.
% We illustrate this algorithm in 
% Based on $C$-separation, each of those statements could be broken down into further conditional independence statements as discussed in Section \ref{subsec:ci_counting}. % Since statements that produce the most conditional independence statements are those with the largest separated sets and smallest conditioning sets.
% However, we can avoid explicitly counting such statements by approximating the 'densest' conditional independence statement by picking one with the largest $|V - n - MB(n)|$, which is the one with the smallest Markov boundary.

% \brit{Anna, we need to change the algo so its output will be subgraphs, to be processed by the greedy algo}
\setlength{\textfloatsep}{2px}
\SetInd{1.0ex}{1.0ex}
\begin{algorithm}[t]
\scriptsize
	\DontPrintSemicolon
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{A causal DAG $\cg$, a number $k$, and a size threshold $\sigma$. }
	\Output{A list of subgraphs.} \BlankLine
  \SetKwFunction{GetMBCIs}{\textsc{GetMBCIs}}

 indivisibles $ \gets \emptyset$\\
  pqueue$ \gets \cg$\\
  \While {|pqueue| $> 0$ and
        $k < $|pqueue| $+$ |indivisibles|\tcp*{\textcolor{blue}{Stop when we have enough components or can't split any more}}}{
        

    subgraph $\gets$ pqueue.pop()\\
    % \tcp*[h]{\textcolor{blue}{Don't consider splitting when there's no \ci\ or graph is too small} \\
    \If{ subgraph is a complete graph or |subgraph| $\leq \sigma$ \tcp*{\textcolor{blue}{Don't consider splitting when there's no \ci\ or graph is too small}}}
    {
        indivisibles.put(subgraph)\\
        continue\\
    }
    sgMB $\gets$ subgraph.\GetMBCIs(subgraph) \tcp*{\textcolor{blue}{Split the graph}}\\
    XZComponent $\gets$ subgraph with the smallest
        Markov boundary and its node\\
    YComponents $\gets$ weakly connected components
         in subgraph $\setminus$ XZComponent\\
    partitions $\gets$ XZcomponent + YComponents\\
    testAcyclicityGraph $\gets$ subgraph$/$partitions\\
    \While{ testAcyclicityGraph.HasCycles \tcp*{\textcolor{blue}{Ensure acyclicity of the cut}}}
    {
    frontierXZ $\gets$ XZComponent.nodes with an edge
    connecting to node out of the component\\
    frontierY $\gets$ YComponents.nodes with an edge
          connecting to a node in XZComponent\\
    chosenNode $\gets$ random(frontierXZ $\cup$ frontierY)\\
    \If{ chosenNode $\in$ XZComponent}
       { move chosenNode to a random YComponent it
            has an edge to\\
            }
    \Else{
        move chosenNode to XZComponent\\
      partitions $\gets$ XZComponent $\cup$ YComponents\\
      testAcyclicityGraph $\gets$ subgraph $/$ partitions\\
    }
    }
     pqueue.put(partitions) \tcp*{\textcolor{blue}{Enqueue new subgraphs}}\\
}
  % partition $\gets$ pqueue + indivisibles\\
  % $\mathcal{G}' \gets \mathcal{G}/$partition\\
  % \Return $\mathcal{G}'$\\
  \Return pqueue + indivisibles
 
\caption{Markov Boundary Partitioning Algorithm}\label{algo:mb_algo}
\end{algorithm} 


\subsection{The Full CAMBA Algorithm}
\label{subsec:camba}

We are now ready to introduce our Causal Acyclic Markov-Boundary (CAMBA) Algorithm. In a nutshell, this algorithm uses the Markov Boundary Partitioning algorithm to split the input causal DAG into smaller subsets, then uses the Greedy Search algorithm to summarize each of the subgraphs.

The algorithm also employs two heuristic initial node-merging passes to capture high-value, low-cost clustering choices before entering the partitioning phase.

\paragraph{\bf Merge Heuristics}
As a pre-processing step, we merge nodes with the same children and parents, as well as nodes connected along a non-branching path of nodes, each with at most one parent and one child.
% an isolated path. % or string \brit{Anna, what is a string of nodes?} of nodes.
Merging nodes with the same parents and children has the advantage of minimizing risk of losing other CI statement upon compression. Only the CI statements between the merged nodes are lost, which would have happened anyway between any arbitrary merged nodes. This type of merge often results in the least total loss of \ci\ among all possible merges. Similarly, merging nodes along a non-branching path in the graph does not impact CI statements between other nodes in the graph. All paths that pass through the merged nodes remain intact, and no new paths are introduced, thereby preserving \ci.


\vspace{3mm}
% \brit{Anna, describe here the full \algoName\ algorithm, change it so it will call the partitioning algo to get the subgraphs, then run the greedy search on each subgraph, and finally merge it all into a single quotient graph. }
% \anna{as seen in algorithm \ref{algo:camba}, \algoName\ starts with heuristic merging, then partitions the graph into subgraphs with the markov boundary partitioning, then runs greedy search on each subgraph. based on the split or merge choices made in this algorithm, the final quotient graph is formed and reutnred ot the user.}
\algoName\ (reproduced in Algorithm \ref{algo:camba}) begins with heuristic merging, then uses Markov boundary partitioning (Algorithm \ref{algo:mb_algo}) to partition the graph into subgraphs small enough to run Greedy search (Algorithm \ref{algo:greedy_search}) on each of them, and lastly uses the final partitioning to form the output quotient graph. If at any point the algorithm meets the exact $k$ required nodes, no further refinement is needed and the algorithm can exit early by forming an output quotient graph with the partition it has so far.


\setlength{\textfloatsep}{2px}
\SetInd{1.0ex}{1.0ex}
\begin{algorithm}[t]
\scriptsize
	\DontPrintSemicolon
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\LinesNumbered
	\Input{A causal DAG $\cg$, and a number $k$. }
	\Output{A quotient causal DAG $\qg$ with no more than $k$ nodes.} \BlankLine
  \SetKwFunction{HeuristicMerges}{\textsc{HeuristicMerges}}
   \SetKwFunction{MarkovBoundaryPartitioning}{\textsc{MarkovBoundaryPartitioning}}
   \SetKwFunction{GreedySearch}{\textsc{GreedySearch}}
 

  $\qg \gets \HeuristicMerges(\cg, k)$\\
  \If {|$\qg$.nodes| $\leq k$}
    {return $\qg$\\
    }
  $Q \gets \MarkovBoundaryPartitioning(
      \qg, k$)\\
      $\ell \gets 0$ \\
      partition $\gets []$ \\
\While{$|Q| > 0$ \tcp*{\textcolor{blue}{$Q$ is sorted smallest first}}} {
    subgraph \gets $Q$.pop() \\
    $\qg \gets \GreedySearch$(subgraph, $\frac{k-\ell}{|Q|}$)) \\
    partition.add($\qg$.partition) \\
    $\ell \gets \ell + |\qg$.partition|
}
  \Return $\cg / $ partition

 
\caption{The \algoName\ Algorithm}\label{algo:camba}
\end{algorithm} 







\paragraph*{\bf Time Complexity}
Let $n$ be the number of nodes in the input causal DAG $\cg$, $d$ the density of $\cg$, $e$ to indicate an exponential and $log$ to indicate a logarithm, and $m$ the internally-set maximum size of a subgraph where the partitioning algorithm stops and the greedy algorithm runs.
The heuristic merges algorithm takes $O(n^2)$;
% the Markov boundary enumeration takes $O(nd)$,
the Markov partitioning algorithm takes $O(nd*log(n))$; and 
the Greedy Search takes $O(md)$ plus the fixpoint $C$-separation algorithm $O(e^m)$.
We find that the overall time complexity of the CAMBA algorithm is $O(n^2+nd*log(n)+mde^m)$. % where $m$ is the internally-set maximum size of a subgraph where the partitioning algorithm stops and the greedy algorithm runs.
% \brit{what are n, nd, e and mde? we can improve that if we use parallelism right? to run the greedy search in parallel}
% \anna{i think parallel is considered already; for example, greedy starts with an initial ci list based on markov boundary which is md time, and then runs the csep algorithm on top of that initial list}
% \anna{n = number of nodes, d = density (proxy for how large markov boundaries are), and e is the exponential}
% When $n >> m$, we realize an optimistic $O(n^2)$ runtime; otherwise, we find a worst-case exponential bound with $O(e^m)$.


\paragraph*{\bf Limitations}
Our \algoName\ algorithm generates a quotient causal DAG with a maximum of $k$ nodes. However, it does not guarantee that the resulting quotient DAG will have the highest count of \ci. Despite this, our experimental results demonstrate its effectiveness in practice, even for large input causal DAGs. 

\subsection{Handling Mixed Graphs}

% while a common graph input for causal inference is a causal DAG, other graph representations are also used when a full causal dag is not retrievable -- especially causal discovery algorithms like pc and lingam
While one dominant form of domain knowledge graph input for causal inference is the causal DAG, other graph representations are also used when a full causal DAG is not retrievable, say, by a causal discovery algorithm.
% \mike{It seems very odd to me to describe the results of causal discovery as a “quotient causal DAG”. It hasn’t undergone a purposeful summarization process, as our algorithm performs.}
% % we previously discussed quotient causal dags -- it turns out that these can also be fed into our algorithms without issue to be summarized further
% Our algorithms can further shrink input quotient causal DAGs without modification; however, % , and more causal graph representations can be accommodated with some modification.
Many of these graph representations are referred to as \textit{mixed graphs} due to their inclusion of undirected, bidirected, and other types of edges \cite{chickering2002optimal, perkovic2020identifying}.

% we look at a particular kind of mixed graph which contains undirected edges: partially directed acyclic graphs (PDAGs) and completed partially directed acyclic graphs (CPDAGs)
In this work, we explore a type of mixed graph which contains undirected edges: completed partially directed acyclic graphs (CPDAGs).
% since multple DAGs can hold the same set of conditional independence statements, markov equivalence classes of graphs are representations of groups of causal graphs which share the same properties
Since multiple possible causal DAGs can emit the same set of conditional independence statements discernable from the data, causal discovery methods can emit Markov equivalence classes of graphs, which are representations of groups of causal graphs that share those same properties.
% a PDAG, or chain graph, is a graph that contains both directed and undirected edges that does not contain directed cycles -- this could be interpreted as a graph equivalence class where each directed edge maps to a directed edge of a DAG in the equivalence class, and undirected edge maps to an either-direction directed edge
% a completed PDAG is a \textbf{unique} PDAG.
CPDAGs are graphs which contain both directed and undirected edges without directed cycles---these graphs uniquely represent equivalence classes where each directed edge maps to a directed edge on all compatible DAGs in the equivalence class, and undirected edges map to compatible DAGs with edges oriented in either direction \cite{chickering2020statistically, perkovic2020identifying}.
% algorithms like pc and ges output graph equivalence classes in this way
Causal discovery algorithms like PC \cite{spirtes2000causation} and GES \cite{chickering2002optimal} provide CPDAGs as output.

% we accept such graphs in our algorithm by pre-processing the PDAG or CPDAG into a quotient causal DAG to feed in to the aforementioned algorithms, akin to 'ordered blocking' as in [].
We can accept CPDAGs as input to our algorithm by preprocessing the CPDAG into a quotient causal DAG to be used as an input graph for further summarization, as detailed in Algorithm \ref{algo:cpdag_preprocessing}; this scheme is akin to being an inverse version of \cite{lauritzen_chain_graphs} proposed for \textit{constructing} chain graphs (which are non-unique PDAGs) % and \cite{heskes2020causal} proposed for constructing a partial ordering of causal variables.
and can be thought of as graph condensation for \emph{chain graph} components, rather than strongly connected components.

\begin{algorithm}[t]
\DontPrintSemicolon
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\LinesNumbered
\Input{A causal CPDAG $\mathcal{G}_P$.}
\Output{A quotient causal DAG $\qg$.} \BlankLine

$\mathcal{G}_P` \gets \mathcal{G}_P$ \\
Remove all directed edges from $\mathcal{G}_P`$ \\
$\mathcal{P} \gets$ Connected Components of $\mathcal{G}_P`$ \\
$\qg \gets \mathcal{G}_P / \mathcal{P}$ \\
\Return $\qg$
 
\caption{Preprocessing CPDAGs for Causal Graph Summarization}\label{algo:cpdag_preprocessing}
\end{algorithm}

% further work can explore the applicability of pdag2dag etc.
Further work can explore the applicability of other conversion methods between causal DAGs and mixed graphs like CPDAGs \cite{chickering2002optimal, chickering2020statistically}, PDAGs \cite{dor1992simple}, and other representations.


% \brit{here we need to add the extension for mixed graphs, as a pre-processing step for the algorithm, and explain why this is necessary. }

% i think to _handle_ mixed graphs it would mean that we can feed in a mixed graph, transform it into a causal DAG for the algorithm to summarize, and then (possibly) transform it back to a mixed summary graph that's useful for the end user somehow

% what type of mixed graph would be useful to look at?
% we're looking only at graphs where bidirectional edges mean an undetermined edge direction

% some causal discovery methods output mixed graphs
% which are graphs that contain edges which are different: bidirectional edges!
% due to the ubiquity of these methods and utility of representing causal ambiguity in these types of outputs, we feel that it's important for this work to address this domain

% we remedy this as a preprocessing step by introducing a 'latent factors' node
% given any arbitrary node pair a and b with a bidirectional edge between them, we replace the edge with two edges from the 'latent factors' node to node a and node b.
% in the summarization task, we modify the desired summary size and semantic constraints to ensure that this node will not be merged with other nodes
% after summarization, the bidirectional edges can be re-introduced
% we can (?) demonstrate that there will be no new cycles that would be introduced ???

% alternatively, we can merge all nodes that contain bidirectional edges between them into a condensed graph before starting the summarization task
% that said, the set of valid summarization sizes is narrower
% future work can focus on fully extending this algorithm to work with mixed graphs

==> big-case-study.tex <==
\subsubsection{The utility of the summary causal DAGs for human verifiability}
We evaluate the effectiveness of summary causal DAGs in refining the input causal model. In a case study, we demonstrate that the summary DAG facilitates the detection of errors (such as missing and redundant edges) in the input causal DAG more effectively than directly examining the input causal DAG (which may be overwhelming to the user). This study underscores that causal DAG summarization is valuable not only for reliable causal inference but also for validating the input causal DAG efficiently. 

In particular, we will take a closer look at the \redshift{} dataset. Unlike the illustrative, manually constructed graph of Figure~\ref{fig:example_causal_dag}, which contained 23 edges, the automatically-derived causal DAG for this dataset contains 55 edges and is shown in Figure~\ref{fig:redshift_big_causal_dag}. Verifying the correctness of each individual edge in this DAG is overwhelming for a human user. However, employing \algoName\ with $k = 5$ leads to the much more readily accessible DAG shown in Figure~\ref{fig:redshift_big_causal_dag_summary}, containing only 10 edges. 

In this smaller DAG, a suspicious edge becomes readily apparent: the edge leading from $\textbf{A} = $ \{\verb|Result Cache Hit|, \verb|Plan Time|, \verb|Lock Wait Time|\} to $\textbf{B} = $ \{\verb|Returned Rows|, \verb|Returned Bytes|\}. Intuitively, the amount of data a query returns is not causally affected by execution-related features like the time the query had to wait for locks. This prompts a closer investigation of the edges in Figure~\ref{fig:redshift_big_causal_dag} that originate in a node in $\textbf{A}$ and end at a node in $\textbf{B}$, which uncovers three possibly redundant edges: from \verb|Lock Wait Time| to each of \verb|Returned Rows| and \verb|Returned Bytes|, as well as from \verb|Result Cache Hit| to \verb|Returned Bytes|. These edges can then be removed from the graph. Leveraging the summary provided by \algoName\ allowed us to quickly focus on 3 questionable edges instead of verifying all 55.


\markos{I can also talk about why GPT added these 3 edges in the first place if we want - it's because it thinks that returned bytes and returned rows refer to results across queries, so anything that speeds queries up (less lock waiting, more cache hits) will increase the number of executed queries so also the total bytes returned}







\begin{figure}
\centering

 \scriptsize
       \begin{tikzpicture}[
    every node/.style={
        minimum size=0.5cm, % Adjust the size as needed
        font=\bfseries, % Make the font bold
        align=center, % Align text in the center
         text width=0.8cm % Set text width for wrapping
    },
    vertex/.style={draw, circle}
]
\clip (-2,2.3) rectangle (6.9, -6.7);


\node[vertex] at (0,0) (query_template) {\scriptsize Query\\Template};
\node[vertex] at (1.5,0) (returned_rows) {\scriptsize Returned\\Rows};
\node[vertex] at (3,0) (returned_bytes) {\scriptsize Returned\\Bytes};

\node[vertex] at (0,-1.5) (num_joins) {\scriptsize Num\\Joins};
\node[vertex] at (1.5,-1.5) (num_tables) {\scriptsize Num\\Tables};
\node[vertex] at (3,-1.5) (num_columns) {\scriptsize Num\\Columns};
\node[vertex] at (4.5,-1.5) (result_cache_hit) {\scriptsize Result\\Cache\\Hit};

\node[vertex] at (0,-4) (compile_time) {\scriptsize Compile\\Time};
\node[vertex] at (1.5,-4)(planning_time) {\scriptsize Plan\\Time};
\node[vertex] at (3,-4)(lock_wait_time) {\scriptsize Lock\\Wait\\Time};
\node[vertex] at (4.5,-4) (execution_time) {\scriptsize Exec.\\Time};

\node[vertex] at (2.25,-5.5) (elapsed_time) {\scriptsize Elapsed\\Time};


\draw[->] (num_tables) to[out=45, in=150] (result_cache_hit);
\draw[->] (num_tables) to[out=-60, in=90] (elapsed_time);
\draw[->] (num_tables) -- (execution_time);
\draw[->] (num_tables) -- (returned_rows);
\draw[->] (num_tables) -- (returned_bytes);
\draw[->] (num_tables) -- (compile_time);
\draw[->] (num_tables) -- (planning_time);
\draw[->] (num_tables) -- (lock_wait_time);
\draw[->] (num_tables) -- (query_template);
\draw[->] (query_template) to[out=45, in=90, looseness=0.95] (result_cache_hit);
\draw[->] (query_template) to[out=180, in=180, out looseness=0.7, in looseness=1.5] (elapsed_time);
\draw[->] (query_template) to[out=-135, in=-90, in looseness=1.8, out looseness=3] (execution_time);
\draw[->] (query_template) -- (returned_rows);
\draw[->] (query_template) to[out=45, in=135, looseness=0.9] (returned_bytes);
\draw[->] (query_template) to[out=180, in=180, looseness=0.5] (compile_time);
\draw[->] (query_template) to[out=180, in=135, in looseness=1.5, out looseness=1.2] (planning_time);
\draw[->] (query_template) to[out=-135, in=290, in looseness=2, out looseness=3.5] (lock_wait_time);
\draw[->] (query_template) -- (num_columns);
\draw[->] (query_template) -- (num_joins);
\draw[->] (num_columns) -- (result_cache_hit);
\draw[->] (num_columns) to[out=-120, in=90] (elapsed_time);
\draw[->] (num_columns) -- (execution_time);
\draw[->] (num_columns) -- (returned_bytes);
\draw[->] (num_columns) -- (compile_time);
\draw[->] (num_columns) -- (planning_time);
\draw[->] (num_columns) -- (lock_wait_time);
\draw[->] (num_joins) to[out=135, in=60, out looseness=2, in looseness=1.5] (result_cache_hit);
\draw[->] (num_joins) to[out=180, in=180, in looseness=2] (elapsed_time);
\draw[->] (num_joins) -- (execution_time);
\draw[->] (num_joins) -- (returned_rows);
\draw[->] (num_joins) -- (returned_bytes);
\draw[->] (num_joins) -- (compile_time);
\draw[->] (num_joins) -- (planning_time);
\draw[->] (num_joins) -- (lock_wait_time);
\draw[->] (result_cache_hit) to[out=0, in=0, out looseness=0.8, in looseness=1.5] (elapsed_time);
\draw[->] (result_cache_hit) -- (execution_time);
\draw[->] (result_cache_hit) -- (returned_bytes);
\draw[->] (result_cache_hit) -- (compile_time);
\draw[->] (result_cache_hit) -- (planning_time);
\draw[->] (planning_time) -- (elapsed_time);
\draw[->] (planning_time) to[out=-45, in=-120] (execution_time);
\draw[->] (planning_time) -- (compile_time);
\draw[->] (planning_time) -- (lock_wait_time);
\draw[->] (compile_time) -- (elapsed_time);
\draw[->] (compile_time) to[out=-90, in=-90, looseness=1.3] (execution_time);
\draw[->] (lock_wait_time) -- (elapsed_time);
\draw[->] (lock_wait_time) -- (execution_time);
\draw[->] (lock_wait_time) to[out=-45, in=55, out looseness=4, in looseness=4.5] (returned_rows);
\draw[->] (lock_wait_time) to[out=-45, in=60, out looseness=3.5, in looseness=3.2] (returned_bytes);
\draw[->] (returned_rows) to[out=45, in=0, looseness=2.5] (elapsed_time);
\draw[->] (returned_rows) to[out=45, in=0, out looseness=2, in looseness=1.1] (execution_time);
\draw[->] (returned_rows) -- (returned_bytes);
\draw[->] (returned_bytes) to[out=0, in=0, looseness=2.2] (elapsed_time);
\draw[->] (returned_bytes) to[out=0, in=0, out looseness=1.3, in looseness=1.05] (execution_time);
\draw[->] (execution_time) -- (elapsed_time);

%\draw [brown] (current bounding box.south west) rectangle (current bounding box.north east);
%\draw[gray,step=1] (-2,2) grid (8, -8);



\end{tikzpicture}
\caption{Automatically-derived causal DAG for \redshift} \label{fig:redshift_big_causal_dag}
\end{figure}


\begin{figure}
\centering

 \scriptsize
       \begin{tikzpicture}[
    every node/.style={
        minimum size=1cm, % Adjust the size as needed
        font=\bfseries, % Make the font bold
        align=center, % Align text in the center
    },
    vertex/.style={draw, circle}
]

\clip (-1.7,1.5) rectangle (3.5,-4);

\node[vertex] at (0,0) (Temp) {\scriptsize Query\\Template,\\ Num Columns,\\ Num Joins}
\node[vertex] at (2, 0) (Returned) {\scriptsize Returned\\Rows,\\Returned\\Bytes}
\node[vertex] at (1,-1.5) (Tables) {\scriptsize Num\\Tables}
\node[vertex] at (0,-3) (Result) {\scriptsize Result\\Cache Hit,\\Plan Time,\\Lock Wait\\Time}
\node[vertex] at (2, -3) (Elapsed) {\scriptsize Elapsed\\Time,\\Exec.Time,\\Compile\\Time}

\draw[->] (Tables)--(Result)
\draw[->] (Tables)--(Elapsed)
\draw[->] (Tables)--(Returned)
\draw[->] (Tables)--(Temp)
\draw[->] (Temp)--(Result)
\draw[->] (Temp) to[out=45, in=45, looseness=1.7] (Elapsed)
\draw[->] (Temp)--(Returned)
\draw[->] (Result) -- (Elapsed)
\draw[->] (Result) to[out=135,in=135, looseness=2] (Returned)
\draw[->] (Returned) -- (Elapsed)


%\draw [brown] (current bounding box.south west) rectangle (current bounding box.north east);
%\draw[gray,step=1] (-2,2) grid (8, -8);



\end{tikzpicture}
\caption{\algoName-generated summary of Figure~\ref{fig:redshift_big_causal_dag} for $k=5$.} \label{fig:redshift_big_causal_dag_summary}
\end{figure}

==> intro_old.tex <==
\section{Introduction}

Causal inference enables researchers and analysts across economics~\cite{}, sociology~\cite{}, medicine~\cite{}, and more~\cite{}, to uncover cause-and-effect relationships and evaluate the effects of medical~\cite{}, behavioral~\cite{}, and policy interventions~\cite{}. \anna{TODO: add citations}

To ensure accuracy in causal effect estimation, an appropriate set of confounding variables must be identified to rule out a causal effect calculation distorted by spurious associations \cite{pearl2018book}. Absent full knowledge of underlying data generative processes in most practical situations, Pearl's causal model \cite{pearl2000models} enables adequate confounding variable identification using \textit{causal graphs} which represent causal relationships among variables in a system.

However, % in much of causal inference literature these causal graphs are often assumed to exist a priori or are ground truth graphs retrieved from domain expertise;
if the causal graphs are incorrect, the causal conclusions cannot be guaranteed to be correct.
Literature in causal discovery and structure learning~\cite{glymour2019review} recognizes the difficulty of recovering causal graphs from data alone, which is exacerbated as data and dimensionality increase. Data integration allows causal analysts to include an expansive pool of potential confounding variables but can result in causal graphs that are structurally complex beyond human verifiability~\cite{youngmann2023causal}.
A reasonable next step is to explore summary graph representations; however, existing state-of-the-art methods~\cite{liu2018graph} do not guarantee to preserve the causal interpretation of the graph and therefore may not be suitable for use in causal inference.

\anna{
add a brief note about dags in the existing literature, this is one study in the health domain -- there's a growing number of them, but they average around 12 nodes each with a density of <50\%; a third contain unobserved variables which integration could help with and almost a fifth already use summarized graphs where some nodes represent multiple causal variables~\cite{tennant2020dagsinhealth}
to allow scientists to include such dags in academic literature we need a way to communicate large complex causal systems in a simple way.
}
% tennant2020dagsinhealth - avg 12 node graphs with 29 edges; "37% (n = 53) of the DAGs included unobserved variables, 17% (n = 25) included ‘super-nodes’ (i.e. nodes containing more than one variable)"

This paper tackles such challenges by formulating a \textit{causal graph summarization} objective, where summaries must strike a balance between simplifying the graph for improved comprehensibility and retaining causal information necessary for reliable inference. Achieving this goal requires an approach that acknowledges the distinctive semantics of causal graphs, setting them apart from other types of graphs like transportation~\cite{} or social networks~\cite{}.
% \anna{everything above is anna's attempt at a revision based on mike's awesome comments on babak's stellar draft; i feel a bit self-conscious commenting out all of babak's text, so if you want to keep reading jump to the example and the paragraphs after}
To illustrate our proposed approach, we provide a concrete example that showcases its effectiveness:

\begin{comment}
\mike{(referring to this paragraph) Too much. We can introduce in one or two sentence.}
%% importance of causal inference
Causal inference, a critical aspect of empirical research, holds immense importance across various disciplines, including economics, sociology, and medicine. It serves as a powerful tool for examining cause-and-effect relationships, particularly in evaluating the effects of interventions. Researchers employ causal inference to address questions like the impact of a specific educational program on student performance, independent of socioeconomic factors, or the effectiveness of a new drug treatment for a disease, regardless of other concurrent therapies. By employing rigorous methodologies, causal inference enables economists to gauge the actual influence of policy interventions on economic outcomes, helps healthcare professionals identify the most effective treatments, and assists social scientists in deciphering the true effects of social programs. By uncovering the causal mechanisms at work, this approach empowers decision-makers with evidence-backed insights to drive positive changes and inform future interventions.
\anna{(attempt at a revision:) Causal inference enables researchers and analysts across economics, sociology, medicine, and more, to uncover cause-and-effect relationships and evaluate the effects of medical, behavioral, and policy interventions.}

%%% causal graphs
\mike{(referring to the next two paragraphs) Again we can compress substantially. Basically: Pearl model is standard and it needs a graph. If your graph is wrong then your causal answer will be wrong. Lots of work exists on how to build these graphs.}
To ensure the accurate estimation of causal effects and avoid the pitfalls of confounding bias, it is crucial to carefully consider the presence of confounding variables. These variables have the potential to influence both the exposure and the outcome, leading to distorted associations between them \cite{pearl2018book}. A key aspect of addressing confounding bias lies in understanding the underlying data generative process and identifying an appropriate set of confounding variables. Causal graphs have proven to be powerful tools for representing this background knowledge. By visually depicting the causal relationships among variables, causal graphs help capture the complex interplay between factors and provide a systematic framework for understanding cause-and-effect relationships~\cite{pearl2000models}. By leveraging these graphical representations, researchers can better account for confounding variables, enhancing the reliability and validity of their analysis of causal effects.

Furthermore, causal models prove to be essential in various ML tasks, extending their usefulness beyond causal inference. They play a significant role in promoting fairness by addressing biases that may be present in data and algorithms, ensuring equitable outcomes~\cite{XXX}. Causal models also facilitate domain adaptation, enhancing the transferability of models across different contexts, which is crucial for achieving robust and effective performance~\cite{XXX}. Moreover, in the domain of reinforcement learning, causal models enable efficient decision-making by capturing the causal relationships between actions and outcomes, guiding the learning process to make optimal choices based on interactions with the environment~\cite{XXX}.
\babak{Please add citations}
\anna{
(attempt at a revision for the above two paragraphs and the below two paragraphs:) To ensure accuracy in causal effect estimation, an appropriate set of confounding variables must be identified to rule out a causal effect calculation distorted by spurious associations \cite{pearl2018book}. Absent full knowledge of underlying data generative processes in most practical situations, Pearl's causal model \cite{pearl2000models} enables adequate confounding variable identification using \textit{causal graphs} which represent causal relationships among variables in a system.
However, % in much of causal inference literature these causal graphs are often assumed to exist a priori or are ground truth graphs retrieved from domain expertise;
if the causal graphs are incorrect, the causal conclusions cannot be guaranteed to be correct.
Literature in causal discovery and structure learning~\cite{glymour2019review} recognizes the difficulty of recovering causal graphs from data alone, which is exacerbated as data and dimensionality increase. Data integration allows causal analysts to include an expansive pool of potential confounding variables but can result in causal graphs that are structurally complex beyond human verifiability~\cite{youngmann2023causal}.
A reasonable next step is to explore summary graph representations; however, existing state-of-the-art methods~\cite{liu2018graph} do not guarantee to preserve the causal interpretation of the graph and therefore may not be suitable for use in causal inference.
}

Causal graphs, despite their significance, often pose a challenge to analysts due to their unavailability or the inherent difficulty in fully recovering causal graphs from data alone~\cite{glymour2019review, pearl2018book}. \mike{Hard to know if it’s inherent so I would delete. But it’s hard certainly} This challenge becomes particularly pronounced as data complexity and dimensionality increase. \mike{(referring to the rest of the paragraph) Not sure what this text is trying to do.
Are you just saying the graph might have to be big?  If so then we should cite papers with big graphs, if possible.} In practical situations across various fields such as healthcare, climate science, and business analytics, the integration of available data with external or interval datasets is necessary to incorporate all potential confounding variables, which further complicates graph construction. For example, in healthcare, the integration of electronic health records, genomic data, and patient feedback results in a high-dimensional data environment. Climate scientists encounter the challenge of merging diverse datasets encompassing elements like carbon emissions and temperature records. Similarly, in business analytics, integrating data from internal databases such as sales records or customer interactions with external datasets like market trends or economic indicators is crucial. \mike{In general we can be a lot more succinct} Furthermore, the involvement of domain experts adds to the complexity, particularly in high-dimensional settings. These practical examples highlight the intricacies of constructing causal graphs and emphasize the need for innovative solutions to create meaningful graphs in high-dimensional scenarios.



\mike{(referring to this paragraph) i think the text is trying to argue for this work from first principles. But it is leading the text to be too high level. 
Instead just say that sometimes we have a causal graph that’s too big (possibly because it’s generated automatically).  A big graph is bad because X. You might think we could just summarize the graph but we can’t because the resulting graph will mess up the causal interpretation.  The reason the interpretation gets messed up is because we fail to preserve causal independencies.}
Furthermore, our current knowledge base often falls short in providing a comprehensive understanding of the underlying causal models, particularly in complex high-dimensional scenarios involving numerous variables. Despite having some contextual or temporal information, establishing the relationships between each variable pair can be an exhaustive endeavor. Given the significant risks associated with drawing incorrect inferences from a mis-specified causal graph, it becomes crucial to explore the possibility of using a simpler, coarser representation that not only facilitates easier elicitation and verification of information from domain experts but also effectively addresses specific causal queries. The development of such a representation has the potential to revolutionize the approach to handling high-dimensionality in causal inference, simplifying the process while maintaining accuracy and depth of information.


This paper tackles the complex challenges associated with high-dimensional causal graphs by introducing the concept of causal graph summarization as a viable solution. Our objective is to strike a balance between simplifying the graph for improved comprehensibility while retaining essential causal information necessary for reliable inference. Achieving this goal requires a distinct approach that acknowledges the distinctive semantics of causal graphs, setting them apart from other types of graphs like transportation or social networks. To illustrate our proposed approach, we provide a concrete example that showcases its effectiveness.
\anna{(admittedly weak attempt to shrink this paragraph:) 
This paper tackles such challenges by formulating a \textit{causal graph summarization} objective, where summaries must strike a balance between simplifying the graph for improved comprehensibility and retaining causal information necessary for reliable inference. Achieving this goal requires an approach that acknowledges the distinctive semantics of causal graphs, setting them apart from other types of graphs like transportation or social networks.
}
\end{comment}
% \babak{Here we can provide the example. But it needs to shows the challenges, and your system's input and output as well as its functionality}
\begin{example} \label{ex:jan}
% \mike{Not a bad scenario but should be three sentences.
% There’s a lot of detail here we don’t need. Boil this down into a simple running example and get rid of the rest}
Jan at the US Department of Transportation wants to find out whether any particular US airport causes flight departure delays irrespective of possible covariates like weather and airline business operations. To conduct causal inference, Jan \textit{integrates} a base table of flight departure data with external data sources using state-of-the-art data discovery and integration tools (e.g., \cite{nargesian2018table,zhang2020finding}) and uses a causal discovery tool (e.g., \cite{ramsey2018tetrad,spirtes2000causation}) to automatically construct a causal DAG; overwhelmed with a large, dense graph with many meaningfully overlapping nodes, Jan uses an off-the-shelf graph summarization algorithm~\cite{zhu2016unsupervised}
% \anna{this is the first newer listed algorithm from 2016 included in the 2018 ACM graph summarization survey}
so that a smaller causal graph can be used for inference. With this graph summary in hand, Jan finds a significant causal effect for a number of airports. \anna{and then... maybe does something about it? sends some concerned emails? TODO item for whether we need to include a more significant implication of this choice}

Unbeknownst to Jan, this causal conclusion is erroneous due to the unassuming removal of key confounding variables which the graph summarization method deemed not essential to include in the summary graph. Had Jan used a causal graph summarization method, this would not have happened. As we discuss in Section \ref{subsec:qcg}, such methods would guarantee that re-introduction of confounding bias is not possible.
% \anna{something about how the result is spurious because the graph summarization technique actually removed some key confounding variables which it deemed not useful, despite it being mainly a grouping-based method. if they use a causality-aware method, this would not have happened.}
\begin{comment}
% \anna{user-driven motivation/story for wanting to find actionable insights but not being able to due to both issues with scale and data quality issues that limit causal inference applicability}
% builder of a new airport wants to figure out how to build an effective airport and wanted to understand what interventions would be useful for mainimizing departure delay
% they have the existing flights data
Jan is an analyst in the US Department of Transportation,
looking to conduct a causal analysis to determine the impact that the choice of an airport has on flight departure delay.
Jan has the data detailing flight departures across the country, like the departure airport and flight number, but it's missing key confounding variables, like weather-related attributes including precipitation and airline-related attributes like number of staff members. Jan reasons that these attributes are feasibly related to the phenomenon of interest, but requires more background knowledge of causal relationships to determine which of these variables are confounding variables to account for.
Here, variables missing from the dataset are critical for the analysis to avoid confounding bias. Thus, Jan must \emph{integrate the data} with external data sources %. This is a laborious task,
% typically done
using data discovery and integration tools (e.g., \cite{nargesian2018table,zhang2020finding}). % by skilled programmers---which is often not the case for social or natural scientists. We argue this is the case for many real-life scenarios.
After augmenting the data to include the hundreds or thousands of newly found variables, the next step is determining a sufficient adjustment set of variables to account for confounding bias.
Since Jan does not have the required background knowledge to do that,
%
Jan uses a causal discovery tool (e.g., \cite{ramsey2018tetrad,spirtes2000causation}) to automatically construct a causal DAG and identify the sufficient adjustment set.
%
% However, Mary does not have the required background knowledge to do that.
After letting the tool process all of this newly-augmented dataset to automatically discover a causal DAG that captures the causal relationships in the flight data, \mike{There should be a question the person wants to answer. They get a wrong answer because their graph is poorly summarized} Jan finds that the algorithm suggests an adjustment set of more than 200 individual attributes, many of which are meaningfully overlapping. % and contain missing values.
Incorporating all of the attributes is beyond the computational feasibility of the causal analysis task, and Jan does not have the required background knowledge to determine which subset of those attributes are actually necessary to include in the adjustment set necessary for conducting the desired analysis.
For clarity, an example of the graph Jan wished to have had is presented in Figure \ref{fig:causal_dag}, with the summarized graph involving only two nodes to be included in the adjustment set.
\end{comment}
% \mike{We haven’t gotten to CIs or our complexity results or algorithmic ideas. Also the payoff of Jan using our method is left hanging} \anna{i'd like a bit more clarity/guidance on what it would take to address this comment; my initial reaction is that we'll get too technical too quickly if we introduce this as part of the example. we can mention this in the contributions paragraphs below}
\anna{TODO: does it illustrate the challenges of the domain and functionality of the system? are the system inputs and outputs clear? how do we illustrate the payoff of jan using our method?}
\end{example}


% \babak{Now our focus will be on discussing the specific technical contributions. We need to clearly position in relation to graph summarization techniques.}







\begin{comment}


% explain to a smart but not causal superfan why they would care
% new take on an existing paradigm: graph summarization



% The study of causality focuses on
Scientific progress can be viewed as an exercise in causal analysis:
% Many scientific endeavors boil down to
understanding systems of cause-and-effect relationships which influence some data-generating or observable phenomena.
In practice, many disciplines, including sociology, medicine, and economics \cite{}, commonly study causal mechanisms which are: \begin{enumerate}
    \item \textit{probabilistic}, such as "Are frequent exposures to second-hand smoke related to a different chance of getting lung cancer compared with the general population?" \cite{},
    \item \textit{type-level}, as opposed to singular, as in "If students spend more time studying, do they get better test scores?" rather than "If Joe spends more time studying, would Joe get a better math test grade?" \cite{},
    \item \textit{partially observable},
    where analysts do not assume they have observations of all causal mechanisms contributing to an outcome,
    % as in "Given salary history data of all employees in my company, what are the factors that drive higher compensation?",
    % as in "Given testing performance and salary history data of all teachers in my state, what are the factors that drive a teacher's ability to educate students?",
    as in "How do we study genetic inheritance without full knowledge of which organisms having which genes?" \cite{wright1921treatment},
    and
    \item \textit{high-dimensional}, as in "Given patients' electronic medical records of emergency room and hospital visits, what cause-and-effect relationships about human health can we infer?" \cite{}.
\end{enumerate}
% Further lines of work focus on specialized, domain-specific interpretations of causality, including time-dependency \cite{} and program- or process-encoded \cite{} causality, such as DB causality \cite{} and provenance, which might not be adaptable for general purpose causal analysis.
Knowledge about a collection of causal mechanisms is commonly curated in the form of a \textit{causal graph}; this graph is then broadly distributed in survey papers as a form of communication and used in causal analysis tasks like causal inference. % One such example can be found in Figure \ref{fig:causal_dag}.

Literature in causal inference that build upon Pearl's causal model formally describe how to conduct causal analysis on such causal graphs and resolves limitations with correlative analysis, like confounding bias. Efforts like \cite{ma2022xinsight} % \anna{do something with this Xplainer's XDA thing?} % \anna{cite Xplainer's XDA}
% \anna{revise the flight delays example with causal inference}
illustrate the benefits of conducting \textit{causal} analysis rather than correlative analysis---the insights found in causal analysis can directly translate into actionable interventions. Such interventions---like policy changes, shifts in treatment plans, experiment ideas, and more---provide more promise than correlative insights due to the mitigation of confounding and other biases. With this in mind, we illustrate the perspective of an analyst looking to conduct causal analysis to determine the impact that the choice of airport has on flight departure delay:



As we saw in Jan's scenario, state-of-the-art in causal inference
struggles to scale in both graph size and scope of applicability.
% applicability
Causal graphs suitable for use in causal inference require a number of assumptions which are difficult to demonstrate adherence to in practical settings, including:
% sufficiency
% faithfulness
% markov property
% distributional assumptions
% the data generation process, and lack of unobserved confounders \cite{chickering2002optimal, shimizu2006linear}
sufficiency (there are no unobserved confounders);
faithfulness (the graph captures all conditional independence relations between the variables);
the Markov property (every variable is independent of its non-descendants, given its parents); 
%and
the DAG assumption (the causal graph is a directed acyclic graph);
distributional assumptions (assuming all causal contributions are functionally linear, for example);
and various implicit data modeling assumptions (adequate attribute granularity and a lack of functional dependencies, for example)
% \anna{list out reasons, like high dimensionality of data, column granularity}
\cite{kalainathan2018structural,glymour2019review,chickering2002optimal}.
% graph size
Most causal graphs found in causal inference literature contain around 10 or 20 causal attributes \cite{} which are curated manually or semi-manually \cite{}; while methods are capable of incorporating large populations of study units, often represented as rows in observational relational data, our current methods are not built for high-dimensional datasets with significantly more causal attributes.
% Automated methods may provide the possibility of working with larger graphs for causal inference, but without sufficient guarantees and the means to navigate those larger graphs
% Optimistically, even if causal discovery methods succeed beyond our wildest dreams, we will have vast causal graphs that are difficult for humans to make sense of.
% \anna{illustrate which parts of the example can't be used due to said issues, or whatever the takeaway is for this paragraph}
% However, such assumptions
% may not hold in practice, and therefore limit the applicability of these algorithms.
% Further, such algorithms may not capture causal relations that are not present in the data,
% and ignore semantic and contextual information found in the attribute names and values.

Data summarization has made big data analytics feasible \cite{}; in particular, graph summarization has worked very well for road, social, and computer network analysis \cite{}. To combat the limitations of current causal analysis methods and enable them to scale to high-dimensional datasets, we can endeavor to summarize the graph before use in causal analysis tasks.
However, the state-of-the-art in graph summarization is inadequate for graphs with cause-and-effect relationships.
% \anna{list out reasons, such as semantics of causal edges}
The semantics of an edge in a causal graph differ significantly from, say, that of a road network---summarization by outright edge or node removal would introduce spurious causal information in a causal graph, whereas visualizing a road network would be much faster without drawing the residential side streets. Even when compared with a Bayesian network, the semantics of the directionality of an edge results in different solution spaces for graph summarization.
Consequentially, objectives like minimum description length (MDL), edge minimization, conductance, or flow minimization do not have clear alignment with summarization in the causal graph domain.
% \anna{provide the flight delays example or some other example, exhibits A, B, C where a is the original, b is a BAD summarization, c is an AWESOME one -- merged nodes that are suboptimally. add an example somewhere}
% Even if we found some means of summarizing the causal graph



We endeavor to discern whether causality-specific graph summarization methods could surmount this causal analysis challenge, while preserving critical invariants that enable incorporation into causal analysis with minimal loss of quality.
% \anna{describe the contributions of this paper}

In this work, we present the following contributions:
% \anna{extend each bullet into a paragraph}
\mike{I’d boil these down to 3-4 short paras}
\begin{enumerate}
    \item We formalize the \probName\ problem in which a large causal graph can be summarized for comprehensibility and causal information retention.
    \item We define a structural causal information metric of a summarized graph which does not rely on any information beyond the labeled causal graph.% as the size of the set of conditional independence statements able to be represented in the causal graph.
    \item We introduce $C$-separation, an extension of $d$-separation that operates on quotient causal graphs.
    \item We characterize graph summarization operations that are sound relative to this metric.
    \item We present a naive brute force algorithm to concretely quantify this structural metric for any given causal graph.
    \item We further develop fast, approximate methods to estimate this structural causal information metric.
    \item We present \algoName, our illustrative prototype of a causal graph summarization method, to highlight opportunities for greedy, bottom-up, and top-down causality-specific optimizations.
    \item We demonstrate performance and outcome characteristics of these algorithms on a range of causal analysis scenarios.
\end{enumerate}
\end{comment}

To establish this body of work, in Section \ref{sec:problem} we introduce and formalize the \probName\ problem in which a large causal graph can be summarized for comprehensibility and causal information retention.
% To further concretize the objective, we quantify causal information retention by introducing a structural causal information metric 
Such causal information retention is quantified in Section \ref{sec:csep} through our introduction of a structural causal information metric which depends solely on the labeled causal graph.
To clarify what class of summary graphs can be used for causal inference, we identify the elementary graph operations that are sound relative to this metric; in this manner, we determine what class of graph summarization methods are valid for use in \probName.
In order to evaluate quality among multiple eligible graph summarizations, we introduce $C$-separation, an extension of $d$-separation that operates on such graphs.

% To illustrate the opportunity of causality-aware graph summarization methods, we present
In Section \ref{sec:algorithm}, we present \algoName, our illustrative prototype of a causal graph summarization method, to highlight opportunities for greedy, bottom-up, top-down, and metrics-based causality-specific optimizations. We illustrate identifiability properties which enable the summary graphs to be used in causal inference in Section \ref{sec:identifiability}. Finally, in Section \ref{sec:exp} we demonstrate summarization performance characteristics and causal analysis outcomes of these algorithms on a range of causal analysis scenarios.
\anna{The full technical report will include the proofs.}

% \mike{One problem with intro is that I cannot really say at this point what experiments should be performed to evaluate the work. It means the goals of the work as currently described are too abstract}
% \anna{brit's perspective is that the 'user' problem definition ought to go in the introduction section; 
\anna{somewhere we'd like to be illustrating a bad summarization, describing how the semantic/size constraints and optimization metric of causal information can be useful}
\anna{perhaps compare/contrasting examples of subpar/awesome summarizations and how the constraints/optimization metrics are useful should go somewhere, but there isn't an explicit place for them quite yet...}
% However, unbridled optimization according to that success metric can easily lead to two failure modes:
\mike{Gotta compare against some bad summaries. Also run the query and show that the bad summaries give inaccurate answers}

% hard to analyze
% we offer to summarize
% objective is different from sota
% our contributions
% challenges: what is the ci that are implied, we extended d-separation. how to evaluate, the # is exponential, approximation method. optimized algorithm w/ list of optimizations

==> problem_old.tex <==
% \anna{TODO: write up an informal explanation of the problem definition. something like we want to summarize the graph in a way that allows jan to still run causal queries on causal graphs even though they're big, and we'd like jan to still be able to read and reason about the graph itself. we formulate an optimization problem for causal sturctural information while including size/semantic constraints that a user can set so the graph itself can be comprehended: (give problem definition)}

% \anna{this is pre-existing text, please make use of it}
% Informally, given a causal DAG $\cg$, our goal is to summarize $\cg$ by grouping related variables and only specifying causal relationships between those groups of variables. By doing so, a sufficient adjustment set of variables to be accounted for to answer a causal question of the relationship between an exposure $T$ and an outcome $O$ should still be identifiable from this summarized causal DAG.
% Here, we introduce a few essential prerequisite topics and concretize our goal into a formal problem description.

\begin{problem}[\probName$^\ast$]
\label{partial-causal-graph-summarization-problem}
Given a causal DAG $\cg {=} (\mathcal{V},\mathcal{E})$, a bound $k {<} |\mathcal{V}|$, a semantic similarity measure $sim(\cdot,\cdot)$, and a threshold $\tau$, the goal is to find a \textbf{\emph{summary causal DAG}} s.t:
\begin{itemize}
    \item \textbf{Size Constraint}: the number of nodes in $\qg$ is ${\leq} k$. 
    %, and $\mathcal{G}_P$ maintains $T$ and $O$ in separated single-node clusters. 
    \item \textbf{Semantic Constraint}: the inter-cluster semantic similarity of every cluster of nodes $\boldsymbol{C}$ ($InterSim(\boldsymbol{C})$) in $\qg$ is $\geq \tau$.
    \item \textbf{Objective}: the \textbf{\emph{amount of causal structural information preserved}} is maximized.
\end{itemize}
\end{problem}

\anna{TODO: describe how we cover what summary causal dag is below and that we require this summary to be like this so we can run causal queries on it. and that we'll cover causal structural information later in section 4. coming back to giving an intuition for the problem, compare/contrast examples of subpar/awesome summarizations and describe how the constraints/optimization metrics are useful}
% \anna{brit's perspective is that the 'user' problem definition ought to go in the introduction section; illustrating a bad summarization, describing how the semantic/size constraints and optimization metric of causal information can be useful}
% \mike{We have to show Jan getting a bad answer because summarization is bad. But we haven’t yet said what query is run or how the overlarge graph is generated algorithmically.}

\anna{this is pre-existing text, please make use of it}
% \subsection{Problem Definition}
% \label{subsec:problem}
% \mike{This is the first time the semantic constraint has come up. Bring this idea earlier into the “user problem definition “ of section 2. 
% Also need to give example of how a bad summarization will fail the semantic constraint and give the user trouble.}
Our objective, given a causal DAG $\cg$, is to generate a comprehensible quotient causal DAG $\qg$ that preserves the essential conditional independence information required for answering causal inquiries accurately.
Successful execution of causal queries on a quotient causal DAG requires the retention of all information needed to determine the identifiability of the result of a causal query.
However, unbridled optimization according to that success metric can easily lead to two failure modes: \begin{enumerate}
    \item \textit{Output DAG is identical to the input DAG}: All \ci\ between variables are retained in this scenario, but this means we did not achieve any graph summarization. We, therefore, include \emph{a size constraint} to discourage providing a trivial or unsatisfactory output.
    \item \textit{Output DAG cannot be inspected, interpreted, or verified}: One may provide a quotient DAG that analysts can use to answer causal queries; however, they may struggle to confirm if the quotient causal DAG still retains causal interpretation: namely, whether the graph contains the existence of functional contributions between variables that relate to real-world causal mechanisms. Therefore, we include \emph{a semantic constraint} to ensure that only nodes of similar semantic meaning are clustered together.
\end{enumerate}
We, therefore, define the concept of a semantic constraint imposed on a quotient casual DAG.






\input{quotient-causal-dags}


% \paragraph*{\bf Semantic Constraint}
\subsection{Semantic Constraint}
Semantic similarity is a measure of the likeness of semantic content between two terms \cite{Harispe2015SemanticSF}.
%; a group of concepts with high semantic similarity are considered synonymous, whereas one with low semantic similarity may be meaningfully different and/or contextually very distinct.
Here we concentrate on the semantic similarity of variables (i.e., nodes in a causal DAG). This is evaluated by determining the semantic similarity between their names. We can also consider alternative ways to assess semantic similarity, such as by taking into account the attribute values as well. 
Semantic similarity between variable names can be measured using embedding techniques (e.g.,~\cite{mikolov2013efficient}), ontological relationships (e.g.,~\cite{kashyap1996semantic}), or language models (e.g., ChatGPT). 



We define a semantic constraint using a semantic similarity measure $sim(X,Y)$, which assigns a value in $[0,1]$ to a pair of variables. This will ensure that the resulting quotient causal DAG combines only semantically related variables and restrict the space of all possible partitions of variables.
The semantic constraint sets a threshold on the semantic similarity within each cluster of nodes (i.e., a node in the quotient DAG), referred to as the \emph{inter-cluster semantic similarity}. 
Our framework is capable of supporting inter-cluster semantic similarity defined in multiple ways: e.g., between the closest/farthest nodes within a cluster, or as the average similarity between all the nodes in a cluster.
Let $sim$ denote a similarity measure and $\boldsymbol{C}$ is a cluster of nodes. We denote by $InterSim(\boldsymbol{C})$ the inert-cluster similarity of $\boldsymbol{C}$.  
Given a similarity measure $sim$, a quotient causal DAG $\qg$ and a threshold $\tau$, we say that $\qg$ \emph{satisfies the semantic constraint} if for every node $\boldsymbol{C}$ in $\qg$ (representing a cluster of nodes), $InterSim(\boldsymbol{C}) {\geq} \tau$. 


\begin{example}
Continuing with our example, consider the following semantic similarity values: $sim($\verb|humidity|, \verb|temperature|$) {=} 0.9$, $sim($\verb|precipitations|, \verb|temperature|$) {=} 0.8$,\\ $sim($\verb|precipitations|, \verb|humidity|$) {=} 0.85$, and $sim($\verb|airport|, \verb|temperature|$)$ ${=} 0.6$. Here we define the inter-cluster semantic similarity as the minimum pairwise semantic similarity within the cluster.
Given a semantic threshold of $\tau {=} 0.8$, consider the cluster\\ $\boldsymbol{C}{ =} \{$\verb|precipitations, temperature, humidity|$\}$.
In this case, this cluster satisfies the semantic constraint as\\ $InterSim(\boldsymbol{C}) {=} 0.8 {\geq} \tau$.
By adding the node \verb|airport| to $\boldsymbol{C}$, the updated inter-cluster semantic similarity becomes $InterSim(\boldsymbol{C}) {=} 0.6$, which is below the threshold $\tau$. Thus, including \verb|airport| in $\boldsymbol{C}$ would violate the semantic constraint.  
\end{example}

% \paragraph*{\bf Size Constraint}
\subsection{Size Constraint}
\anna{let's talk about why we introduce a size constraint, referencing some of \href{https://dr.ntu.edu.sg/cris/rp/rp00915}{prof. sourav bhowmick's} work on the cognitive load of graph understanding (i think it's \href{https://dl.acm.org/doi/abs/10.1145/3514221.3522562}{this paper}?)}
% from https://dl.acm.org/doi/abs/10.1145/3514221.3522562
% Low cognitive load. In cognitive psychology, cognitive load refers
% to the used amount of working memory resources (i.e., memory
% demand) [44]. In particular, intrinsic cognitive load is the effort associated with a specific topic (e.g., selecting patterns) and extraneous
% cognitive load refers to the way information or tasks are presented
% to a learner (e.g., presentation of patterns in a VQI) [44]. In the
% context of visual query formulation, cognitive load on a user is
% associated with browsing a pattern set and visually interpreting a
% displayed pattern’s edge relationships to determine if it is useful for
% a query.
% In particular, large graphs overload the human perception
% and cognitive systems, resulting in poor performance of tasks such
% as identifying edge relationships [23, 50]. Consequently, a topologically complex pattern may demand substantial cognitive effort
% (i.e., increase intrinsic cognitive load) from an end user to decide
% if it can assist in her query formulation [24].
The size of the graph
% The Catapult framework [24] comprises of the following three
% steps. First, it partitions a collection of data graphs into a set of
% clusters. Then, it summarizes each cluster into a cluster summary
% graph (CSG) by performing graph closure iteratively on pairs of
% data graphs in the cluster. A closure graph [22] integrates graphs
% of varying sizes into a single graph by inserting dummy vertices
% or edges with a special label such that every vertex and edge is
% represented in it. Finally, it follows a greedy iterative approach
% based on weighted random walks for selecting the canned patterns
% from CSGs based on the aforementioned characteristics. Specifically,
% it exploits a pattern score that incorporates coverage, diversity, and
% cognitive load to associate a score to each candidate pattern. The
% candidate pattern with the largest pattern score and is within a
% user-specified size range (i.e., budget) is greedily selected as the
% best pattern to be added to the canned pattern set of a Pattern Panel.
% The selection process continues until either the required number (a
% user-defined value in the budget) of canned patterns are discovered
% or when no new pattern can be found.
\anna{TODO: write in this paragraph; roughly structured as such:
a size constraint can be on edges, nodes, disk space, minimum description length (cite the MDL paper from sigmod whenever) and is commonly used all over graph summarization
we picked a node based size constraint since it doesn't have any relationship with complexity of the causal system and therefore won't play the role of biasing away/towards any particular density graph
graph complexity (which impacts cognitive load) scales exponentially with node size (cite) so it makes sense to put a cap on that
provide an example where the examples indicate the other constraints can be met but this one might not be met and vice versa
}



% To formally define what it means to design
% causal-aware graph summarization techniques that enable interpretation of, and performant execution of, causal queries,
% We, therefore, formulate our problem as an optimization problem over
% maximal retention of causally-relevant information
% with size and semantic constraints. Formally, 

% \vspace{2mm}
\subsection{Problem Definition}
We are now ready to formulate our problem as an optimization problem, % over maximal retention of causally-relevant information
with size and semantic constraints,
over maximal retention of causal structural information captured in \ci\ retrieved from $C$-separation (see Section \ref{sec:ci_counting}).
 % \anna{i guess we're covering the objective in the next section?}
Formally, 





==> proofs.tex <==
\section{Proofs}

\begin{theorem}[Soundness and completeness of $C$-separation]
\label{c-separation-soundness-completeness}
\anna{describe formally what soundness and completeness would mean here}
\end{theorem}
\begin{proof}
We begin with the premise that some set of nodes $Z$ in the cluster graph $d$-separates some set of nodes $X$ from another set of nodes $Y$ in the cluster graph. These sets of nodes $X, Y, Z$ correspond with sets of nodes $X_u, Y_u, Z_u$ in any underlying compatible causal graph.
In the cluster graph, we know, by the definition of $d$-separation, that $Z$ blocks every path from $x$ to $y$ where $\exists x. x \in X$ and $\exists y. y \in Y$.
% something about how the cluster graph's edges imply possible existing edges between sets of nodes
By definition of a C-DAG, we know that a $C_a \rightarrow C_b$ edge is added in the cluster graph if there exists some $v_a \in C_a$ and $v_b \in C_b$ where $v_a \rightarrow v_b$ in the underlying compatible causal graph. Therefore, the existence of an edge between $C_a$ and $C_b$ would imply that there exists some node in each cluster that has an edge between them. Likewise, the existence of a path between two clusters in a cluster graph implies that there exists at least one path between a node in one cluster to a node in another cluster. However, we don't know which nodes in either cluster are the nodes with the extant path in the underlying compatible causal graph, so we can assume that any node in one cluster might have a possible path to any node in another cluster if there exists a path between the cluster nodes.
% assumption: if we condition on a cluster node we condition on all participating element nodes in the cluster
Knowing what we know about $Z$ in the cluster graph, what does that mean for $Z_u$ in the analogous underlying compatible causal graph?
\anna{need to finish the first draft, then rewrite this}
\end{proof}

\anna{this below is a statement relating d-separation and c-separation, not sure where to put it}
\begin{definition}[$c$-separation]
% cluster graph has X Y Z
% underlying graph has x1 x2 x3... y1 y2 y3... z1 z2 z3...
% if Z d-separates X and Y in cluster graph, then Z d-separates any subset of X from any subset of Y in the underlying graph
If $Z$ $d$-separates $X$ and $Y$ in a cluster graph, then $Z$ $d$-separates any subset of $X$ from any subset of $Y$ in all underlying compatible causal graphs.
\end{definition}
% \anna{this is more of a relationship between d-separation and c-separation; we might want to have a more graphical representation and then discuss how c-sep relates to d-sep in a lemma/theorem/etc.}

\begin{theorem}[Soundness of Vertex Contraction]
% We can prove that the vertex contraction operation does not introduce any new conditional independencies that have not existed in the original causal DAG.
% \anna{fill in what we did (rather than what is currently known): we can prove that algorithms which honor vertex contraction do not introduce new CI's (is sound) though it's reasonable to gather it won't be complete due to loss of CI's once things are merged together, then illustrate the theorem/proof in the proofs section}
\label{vertex-contraction-soundness}
\end{theorem}
\begin{proof}
\end{proof}

\begin{theorem}[Causal Graph Summarization is NP-hard]
\label{problem-is-np-hard}
\anna{describe formally what we mean here}
\end{theorem}
\begin{proof}
\brit{fill in}
\end{proof}
